Heterogeneous Treatment Effects in Social Networks

We study treatment effect modifiers for causal analysis in a social network, where neighbors' characteristics or network structure may affect the outcome of a unit, and the goal is to identify sub-populations with varying treatment effects using such network properties. We propose a novel framework for this purpose that facilitates data-driven decision making by testing hypotheses about complex effect modifiers in terms of network features or network patterns (e.g., characteristics of neighbors of a unit or belonging to a triangle), and by identifying sub-populations for which a treatment is likely to be effective or harmful. We describe a hypothesis testing approach that accounts for a unit's covariates, their neighbors' covariates, and patterns in the social network, and devise an algorithm incorporating ideas from causal inference, hypothesis testing, and graph theory to verify a hypothesized effect modifier. In addition, we develop a novel algorithm for the discovery of network patterns that are potential effect modifiers. We perform extensive experimental evaluations with a real development economics dataset about the treatment effect of belonging to a financial support network called self-help groups on risk tolerance, and also with a synthetic dataset with known ground truths simulating a vaccine efficacy trial, to evaluate our framework and algorithms.

==> graph_patterns.tex <==
\subsection{Finding Candidate Patterns}\label{sec:pattern_mining}
\harsh{done}

We next describe our strategy and algorithm for finding a pattern suspected as being an effect modifier. After finding such a pattern, the TEEM test for effect modifier can be employed to verify whether this pattern is indeed an effect modifier. 

\paratitle{Criterion for suspected patterns:}
We are interested in finding a pattern $\Delta$ that ``separates'' nodes with high CATE from nodes with low CATE. 
Given a network $\set G$ with $n$ nodes, we want to find a pattern that maximizes the difference between between the TE of nodes that contain the pattern in their ego-centric network and the TE of those that do not contain the pattern in their ego-centric network, while accounting for outliers. Formally:
\begin{small}
\begin{eqnarray*}
    \text{arg max}_{\Delta}& \left| \frac{\sum_i \mathds{1}[\Delta \in \set{G}_i] \widehat{\tau}_i}{\sum_i \mathds{1}[\Delta \in \set{G}_i] }   - \frac{\sum_i \mathds{1}[\Delta \notin \set{G}_i] \widehat{\tau}_i}{\sum_i \mathds{1}[\Delta \notin \set{G}_i] }\right|\\
    \text{such that,}&\\
& \left|\frac{\sum_i \mathds{1}[\Delta \in \set{G}_i]}{n} - \frac{\sum_i \mathds{1}[\Delta \notin \set{G}_i]}{n}  \right| \leq \delta
\end{eqnarray*}
\end{small}
where $\Delta$ is a pattern, $\set{G}_i$ is the ego-centric network of node $i$, and the notation $\Delta \in \set{G}_i$ says that $\Delta$ is a subgraph of $\set{G}_i$, and $0 < \delta < 1$. 

Intuitively, this objective function is inspired by the definition of effect modifier in the classic causal inference literature \cite{rubin2005causal} and aims to find a pattern for which the heterogeneity in the CATE is maximized. 
Additionally, we want the pattern to be prevalent in the network. In other words, we want to remove the possibility of the pattern being present in the ego-centric networks of a few outlier nodes with exceptionally high CATEs that contain the pattern, while the rest of the nodes with high CATEs do not contain it. 
This is handled by the constraint over the difference between the nodes whose ego-centric network contains the pattern and those whose ego-centric network does not whose contain the pattern. 
The parameter $\delta$ can be chosen according to the desired sensitivity to outliers where $\delta = 1$ means that the pattern $\Delta$ can be found in the ego-centric network of a single node, i.e., there is no sensitivity to outliers, and $\delta = 0$ means that the pattern has to be in exactly half of the ego-centric networks.

% to protect the optimal pattern mining against outlier. In other words, we want the pattern to be fairly prevalent and not only present in a fringe cases to ensure generalizability. Thus, we constraint the difference of probabilities of occurrence and absence of the pattern in ego-centric graph. We accommodate this constraint and update the objective to be:
% \begin{eqnarray*}
% \text{arg max}_{\Delta}&& \left| \frac{\sum_i \mathbf{1}[\Delta \in N(i)] \widehat{\tau}_i}{\sum_i \mathbf{1}[\Delta \in N(i)] }   - \frac{\sum_i \mathbf{1}[\Delta \notin N(i)] \widehat{\tau}_i}{\sum_i \mathbf{1}[\Delta \notin N(i)] }\right| \\
% \text{such that,}&&\\
% && \left|\frac{\sum_i \mathbf{1}[\Delta \in N(i)]}{n} - \frac{\sum_i \mathbf{1}[\Delta \notin N(i)]}{n}  \right| \leq \delta
% \end{eqnarray*}
% where $\delta$ is a user-chosen strength of constraint. 


\paratitle{Finding a suspected pattern:}
% This objective function is not differentiable with respect to $\Delta$ and optimizing the above mentioned objective function through a brute-force approach would require iterating over all possible patterns. 
Since the objective function aims to find the pattern $\Delta$ that maximizes the expression, a na\"ive algorithm would iterate over all possible patterns in the network $\set G$, which would require iterating over an exponential number of patterns in $|\set G|$. 

Instead, we propose a greedy approach that eliminates the need to iterate over all patterns. 
Intuitively, the algorithm attempts to find the largest pattern that is found in the ego-centric networks of the nodes with the highest TE, while still satisfying the condition in the optimization problem. 
Algorithm \ref{algo:pattern} gets as input the social network, a list of pairs of nodes and their respective CATEs, the parameter $\delta$ that determines the outlier sensitivity, and a threshold for minimal pattern size $c$. 
It first sorts the nodes by their CATE, sets the initial pattern to be the ego-centric netwrok of the node with the highest CATE, and initializes an index $j$ (lines \ref{l:sort}--\ref{l:index}). 
Next, the algorithm updates the pattern in a while loop that runs as long as the condition in the optimization problem is not satisfied (line \ref{l:while1}). 
It does so by finding the largest common subgraph between the current pattern and the ego-centric network of the next node in the sorted list (function $LCS$ in line \ref{l:lcs1}), and if the updated pattern is larger than the specified threshold, it is updated (lines \ref{l:threshold}--\ref{l:update1}). 
The second while loop considers more nodes from the sorted list and tries to increase the objective expression while also ensuring that the condition in the optimization function is still satisfied (lines \ref{l:while2}--\ref{l:index2}). Finally, it returns the generated pattern in line \ref{l:return-pattern}.

\begin{small}
\IncMargin{1.1em}
\begin{algorithm}[!htb]
	\SetKwFunction{Test hypothesized effect modifier}{Test hypothesized effect modifier}
	\SetKwInOut{Input}{input}\SetKwInOut{Output}{output}
	\LinesNumbered
	\Input{Social network $\set{G}$, a list of pairs $(i, \widehat{\tau_i})$ where $i$ is a node and $\widehat{\tau_i}$ is its estimated TE $L_{\widehat{\tau}}$, outlier sensitivity $\delta$, minimal pattern size $c$}
    \Output{Candidate pattern $\Delta^*$}
	\BlankLine
    
    $S_{\widehat{\tau}} \gets sort(L_{\widehat{\tau}}, by=\widehat{\tau}_i,\text{descending})$\;\label{l:sort}
    $\Delta^* \gets \set{G}_{{S_{\widehat{\tau}}[0][0]}}$\;
    $j \gets 1$\;\label{l:index}
    \While{$\left|\frac{\sum_i \mathds{1}[\Delta^* \in \set{G}_i]}{n} - \frac{\sum_i \mathds{1}[\Delta^* \notin \set{G}_i]}{n}  \right| > \delta$}
    {\label{l:while1}
        $\Delta^{'} \gets LCS(\Delta^*,\set{G}_{S_{\widehat{\tau}}[j][0]})$\;\label{l:lcs1}
        \If{$|\Delta^{'}| > c$}
        {\label{l:threshold}
            $\Delta^* \gets \Delta^{'}$\;\label{l:update1}
        }
        $j \gets j+1$
    }
    \While{$\left|\frac{\sum_i \mathds{1}[\Delta^* \in \set{G}_i]}{n} - \frac{\sum_i \mathds{1}[\Delta^* \notin \set{G}_i]}{n}  \right| \leq \delta$}
    {\label{l:while2}
        $\Delta^{'} \gets LCS(\Delta^*,\set{G}_{S_{\widehat{\tau}}[j][0]})$\;\label{l:lcs2}
        \If{$Objective(\Delta^{'})>Objective(\Delta^{^*})$ and $|\Delta^{'}| > c$}
        {
            $\Delta^* \gets \Delta^{'}$\;\label{l:update2}
        }
        $j \gets j+1$\;\label{l:index2}
    }
    \Return $\Delta^*$\;\label{l:return-pattern}
	\caption{Find suspected pattern}
	\label{algo:pattern}
\end{algorithm}
\end{small}

% \textbf{Greedy algorithm}($\delta$,$c$,$\{\widehat{\tau}_i\}$,$\{i\}$,$\{N(i)\}$):
% \begin{enumerate}
%     \item $s \leftarrow sort(\{i\}, by=\{\widehat{\tau}_i\},\text{descending})$
%     \item $\Delta^* \leftarrow N({s[0]})$
%     \item $j \leftarrow 1$
%     \item while $\left|\frac{\sum_i \mathbf{1}[\Delta^* \in N(i)]}{N} - \frac{\sum_i \mathbf{1}[\Delta^* \notin N(i)]}{N}  \right| > \delta$
%     \begin{enumerate}
%     \item $\Delta^{'} \leftarrow LargestCommonSubgraph(\Delta^*,N({s[j]}))$
%     \item if $|\Delta^*|-|\Delta^{'}| < c$
%     \begin{enumerate}
%         \item $\Delta^* \leftarrow \Delta^{'}$
% % \red{FIX ERROR}
%     \end{enumerate}
%     \item $j \leftarrow j+1$
%     \end{enumerate}
%     \item while $\left|\frac{\sum_i \mathbf{1}[\Delta' \in N(i)]}{N} - \frac{\sum_i \mathbf{1}[\Delta' \notin N(i)]}{N}  \right| \leq \delta$
%     \begin{enumerate}
%         \item $\Delta^{'} \leftarrow LargestCommonSubgraph(\Delta^*,N({s[j]}))$
%         \item if $Objective(\Delta^{'})>Objective(\Delta^{^*})$
%         \begin{enumerate}
%             \item $\Delta^* \leftarrow \Delta^{'}$
%         \end{enumerate}
%         \item $j \leftarrow j+1$
%     \end{enumerate}
%     \item return $\Delta^*$
% \end{enumerate}


% \begin{enumerate}
%     \item Sort the nodes by their TE 
%     \item Start with $p = N(i_{max})$ where $i_{max}$ has the highest treatment effect
%     \item Iterate over the nodes in decreasing order by TE
%     \item For each node $i$, find the largest common subgraph between $p$ and $N(i)$, $p'$
%     \item If $p'$ does not differ from $p$ by more than three edges, assign $p \gets p'$, otherwise, skip
%     \item Stop when $p$ becomes trivial (two edges or less) and return $p$ from the previous step
% \end{enumerate}

% \textcolor{red}{\textbf{Surrogate Objective (Used Earlier)}}
% \begin{eqnarray*}
%     \text{arg max}_{\Delta} \frac{\sum_i \mathbf{1}[\Delta \in N(i)] \mathbf{1}[\widehat{\tau}_i>\tau']}{\sum_i\mathbf{1}[\widehat{\tau}_i>\tau'] }   -  \frac{\sum_i \mathbf{1}[\Delta \in N(i)] \mathbf{1}[\widehat{\tau}_i\leq\tau']}{\sum_i\mathbf{1}[\widehat{\tau}_i\leq\tau'] } 
% \end{eqnarray*}

% \amir{Up to here}

% In this section we use a heuristic algorithm for finding candidate patterns that we can then test whether they are effect modifiers. 

% We find candidate graph patterns using a frequent pattern mining approach. 
% Given a set of nodes with a treatment effect (TE) for each one $\set{V}$, represented as a vector $V.E$, the number of tries to split the nodes into two sets $tries$, the number of simulations $m$, and the sample size $size$, Algorithm \ref{algo:find_patterns} aims to find frequent patterns in the nodes with high TE that are not found in the nodes with low TE. 
% Since TE is continuous, there is no natural splitting point high and low TE. The algorithm starts by choosing the mean of the TE vector as the splitting point of the nodes into those that have TE value higher than the average and those that have TE lower than the average (line \ref{l:mean}). It then enters a loop that runs $tries$ iterations (line \ref{l:tries}) and splits the ego-centric networks of all nodes into two lists: ego-centric networks of nodes that have TE higher than the average, $pos$, and ego-centric networks of nodes that have TE lower than the average, $neg$ (line \ref{l:split}). 
% Then, the algorithm initializes a pattern as the first ego-centric network in the list of nodes that have positive TE and runs $m$ simulations in which it takes a random sample $pos$ of size $size$ and finds the maximum common subgraph in the list of ego-centric networks in the list that includes all networks in the sample and the current pattern (lines \ref{l:simulate}--\ref{l:common}). We do so by employing the ISMAGS algorithm \cite{houbraken2014index}. 
% After finishing the loop, the algorithm uses the procedure \textsc{RemoveCounterfactualEdges} to remove all the edges that do not make the pattern have a non-trivial common subgraph with one of the ego-centric networks in $neg$ (line \ref{l:counterfactual}). 
% This is again performed using the ISMAGS algorithm by iterating over all edges in the pattern, and in each iteration, remove the current edge and checking whether the networks in $neg$ and the new pattern have a non-trivial common subgraph. 
% If the obtained pattern is non-trivial, it is returned (lines \ref{l:non-trivial}--\ref{l:return}), and otherwise, the algorithm chooses a different splitting point by dividing the previous splitting point by $2$ (lines \ref{l:else}--\ref{l:retry}).

% \paratitle{Complexity vs. practical performance}
% Naturally, performing procedures in lines \ref{l:common} and \ref{l:counterfactual} incurs exponential complexity. 
Checking whether the ego-centric network of a node contains a given pattern in lines \ref{l:while1}, \ref{l:while2} and finding the largest common subgraph in two graphs in lines \ref{l:lcs1}, \ref{l:lcs2} incurs exponential complexity in the size of the ego-centric networks as this is equivalent to checking subgraph isomorphism. 
Previous work on this subject has proposed approximation methods and heuristics \cite{?}. 
In our implementation, we have used the ISMAGS algorithm \cite{?}, but other approaches can certainly be plugged in to our algorithm as black-boxes. 

We further employ an optimization that reduces the number of subgraph isomorphisms that need to be considered in each iteration of the two while loops. For nodes that have been considered in previous iterations in the list $L_{\widehat{\tau}}$ and whose pattern $\Delta^*$ was updated in lines \ref{l:update1}, \ref{l:update2}, we do not need to repeatedly check whether their ego-centric network contains $\Delta^*$, since we know that any subsequent pattern will be a subgraph of $\Delta^*$ and therefore, their ego-centric network will contain it as well.  
% We have found that graphs with more than $100$ nodes still pose a challenge. Therefore, we perform the sampling step that, depending on the $size$ and $m$ parameters, significantly decreases the runtime in practice and, even with small sample sizes and relatively small $m$ values, manages to find the correct pattern. 




% We can divide the set of nodes in the network into four sets according to whether they got the treatment and whether they were affected from it (assuming treatment and effect are binary). 
% Then, for each such $i,j$ set where $i$ is the treatment and $j$ is the effect, we convert the labels of all other nodes with different $i,j$ combinations to $X$ standing for `don't cares'. 
% We create a graph list of all ego-centric networks of the nodes in the current combination of $i,j$ and utilize an existing approach (e.g., gSpan \cite{YanH02}) to find the frequent patterns in the list of ego-centric networks that contain the node with the current $i,j$. 
% Finally, we find the set of the common patterns of the sets of $0,0$ and $1,1$ that does not appear in the sets of $1,0$ and $0,1$.


% \amir{Automatically find interesting graph patterns \cite{YanCHY08}. The clever part is finding a good objective function for the patterns. It can be a combination of G-test and measuring the difference in Treatment effect (we also need to get the code and I couldn't find it on Github).}

% \amir{or frequent patterns \cite{ChenYZH07}}

% \amir{Find the graph pattern in the graph. Graph pattern matching may be relevant \cite{SunWWSL12,MaCFHW11,Fan12}}


% \begin{algorithm}[!htb]
% 	\SetKwFunction{Find Graph Patterns}{Find Graph Patterns}
% % 	\SetKwProg{exppattern}{$\texttt{checkGraphPattern}$:}{}{}
% 	\SetKwInOut{Input}{input}\SetKwInOut{Output}{output}
% 	\LinesNumbered
% 	\Input{Social network $\set{G}=(\set{V},\set{E},\set{Z})$, treatment and effect for each unit $v \in \set{V}$, denoted by the vector $V.E$, number of tries to split the nodes into two sets $tries$, number of simulations $m$, sample size $size$}
%     \Output{A network pattern}
% 	\BlankLine
% 	$p \gets mean(V.E)$\;\label{l:mean}
% 	\For{$1,...,tries$}
% 	{\label{l:tries}
% 	    $pos,neg \gets \textsc{SplitByTE}(V.E, p)$\;\label{l:split}
% 	    $pat \gets pos[0]$\;\label{l:init-pattern}
% 	    \For{$1,\ldots, m$}
% 	    {\label{l:simulate}
% 	        $sample \gets \textsc{RandSample}(pos, size)$\;\label{l:sample}
% 	        $pat \gets \textsc{MaxCommonSubgraph}(sample + [pat])$\;\label{l:common}
% 	    }
% 	    $pat \gets \textsc{RemoveCounterfactualEdges}(neg, pat)$\;\label{l:counterfactual}
% 	    \If{$pat.size() > 1$}
% 	    {\label{l:non-trivial}
% 	        \Return $pat$\;\label{l:return}
% 	    }
% 	    \Else 
% 	    {\label{l:else}
% 	        $p \gets \frac{p}{2}$\;\label{l:retry}
% 	    }
% 	}
% 	\caption{Find Network Pattern} 
% 	\label{algo:find_patterns}
% \end{algorithm}
% \harsh{Intuition: interesting patterns are at highly connected nodes - composed of node with similar CATEs. This is the case in favor of looking for cliques.}
% \amir{A more sophisticated algorithm: 1. compute the page rank (or centrality) of each node 2. use MCTS to find the pattern: (a) start with the entire graph and remove one node at each step as in \cite{YuanYWLJ21} (b) the reward for each step will be a combination of the average page ranks of the nodes in the current pattern and the similarity in the CATEs of the nodes in the current pattern (the intuition being that we want the pattern to be composed of central nodes that are similar to each other. We also divide by the size of the pattern since we want compact patterns. (c) the simulation stops when the pattern is empty}

==> intro.tex <==
\section{introduction}\label{sec:intro}
%\amir{Intro on causal inference. Needs to be expanded:}



Causal inference is at the heart of empirical research and principled decision-making in natural and social sciences, and is practically indispensable in epidemiology \cite{robins2000marginal}, clinical research \cite{clinicaltrials2007}, 
public policy \cite{manski2013public}, economics \cite{banerjee2011poor}, and other domains \cite{angrist1996identification,angrist2008mostly}. In causal inference, we go beyond establishing correlation or prediction, and are interested in making causal statements using the concepts of \emph{counterfactuals} and \emph{interventions} about a \emph{treatment} (e.g., administering a vaccine) on some outcome of interest (e.g., not being infected by the targeted disease). While a \emph{randomized controlled trial}, which randomly divides the participating \emph{subjects or units} into \emph{treatment and control groups} at random and evaluates the difference of outcome in these two groups, is considered the gold standard for causal analysis, due to cost or ethics concerns, we often need to rely on \emph{observational causal studies} in data science using collected data under various assumptions as studied in the literature in statistics (e.g., Rubin's potential outcome framework \cite{Rubin1974}) or AI (e.g., Pearl's graphical causal model \cite{pearl2000book}).    
%\red{update last line}.
%\red{another sentence/Rubin-Pearl}
\par
A typical assumption made in the causality literature is {\em no-interference} or \emph{independence} among subjects, %\cite{Rubin1974} \red{correct cite?}, 
meaning that the assigned treatment or the outcome of one subject should \emph{not} affect the outcome of another subject (called \emph{interference} and \emph{contagion} respectively) \red{cite}
%which requires the subject of a study not to have causal interaction with other subjects through ,~
\footnote{Rubin’s potential outcome framework \cite{Rubin1974}, which is a prominent approach for causal inference in statistical studies, relies on the ``\emph{Stable Unit Treatment Value Assumption (SUTVA)}'', which includes the assumption of no-interference.}.
%meaning that treating one subject should not causally influence the outcome of others. 
However, in many studies in social science, the subjects may directly or indirectly interact with each other in different ways and as a result, a subject's outcome (behaviour or states) might be influenced by the %treatment
behavior, states, or characteristics of its social ties in a network, which leads to violation of the no-interference assumption \cite{VanderWeele-book-2013}. 
%\babak{reword the following examples, use examples from social science or add other disciples the the previous sentences} \amir{add one more here}
Examples of such interference include detecting evidence of indirect protection from cholera vaccines when the vaccination rate of individuals in the social network is high \cite{root2011role},
% determining the effect of fake news spreading on elections \cite{bovet2019influence},
or showing that indirect reciprocity inherent in closed triads (triangles) is linked to cooperation between individuals \cite{righi2018social}. 
% since units may be influenced by their neighboring units and by the network structure \cite{everett1990ego,pattison1993algebraic}.
%%%%%%SR -- useful: https://cdn1.sph.harvard.edu/wp-content/uploads/sites/603/2020/07/SNChapter_Book.pdf


This paper focuses on study of {\em treatment effect modifiers~\cite{..} \red{cite Athey?} for causal analysis in a social network}. In a causal study, different subjects may exhibit different levels of response to the applied treatment based on their characteristics, and the effect heterogeneity problem aims to infer this degree %which the applied treatment has different 
of causal effects on different subjects. As an example, one of the key objectives in clinical research is not only to discover effects of %social programs or 
medical treatments at the entire population-level, but also to ascertain 
%{\em treatment effect modifiers} or 
sub-populations (e.g., based on age or previous health conditions) across which the treatment effect differs (e.g., whether a new vaccine is beneficial or harmful).
%is beneficial or harmful. For instance, in medical trials, the goal is to identify sub-populations  for which a treatment  ~\cite{brinkley2010generalized}.  
While different hypothesis tests for the heterogeneity of a population in a study have been proposed in the literature \cite{viechtbauer2007hypothesis, athey2016recursive}, along with a large body of work on testing statistical hypotheses (e.g., \cite{snyder1978hypothesis,xia2017hypothesis,LAROSA201581,shaffer1995multiple,list2019multiple}), such tests 
%are limited to discrete covariates of subjects and 
do not take into account the context of the social network like possible effects of the neighbors' covariates or the network structure on the outcome. On the other hand, while there has been a recent surge of interest in causal inference in social networks~\cite{ogburn2017causal,ogburn2018causal,awan2020almost, DBLP:conf/uai/ShermanS19}, they have not focused on the effect heterogeneity problem. Indeed, reasoning about effect modification and heterogeneity in social networks %is a %very challenging problem. 
poses new conceptual and computational challenges. We illustrate some of these challenges with the following example.   
%i.e., the possible effect of the neighbors' covariates on the outcome and the network structure associated with each unit.

\sudeepa{Edited up to here.}

\cut{
Recently, , as well as to a lesser extent, 
%Much of 
this literature, however, has not addressed the problem of {\em effect heterogeneity}, defined as the degree which different treatments have different causal effects on each subject~\cite{..} \red{cite}. Much literature has focused on detecting heterogeneity and effect modifiers, however, not in the presence of interference and social networks \cite{athey2016recursive}. 
}


%Causal inference exposes insights that are not always evident when using standard data science tools \cite{...}. Thus, it is the standard... 
%Standard causal inference is usually performed over units that can be represented as a single flat table, showing the traits of each unit. 
%\amir{Motivation for working with social networks:}


%However, in more complex realistic scenarios, social networks \cite{sailer1978structural,knoke2019social,wasserman1994social} may better describe additional attributes of the units, such as social relations and interactions \cite{valente2008correlated,granovetter1973strength}. These connections between units are useful in many studies (e.g., vaccine trials \cite{root2011role}, determining the effect of fake news spreading on elections \cite{bovet2019influence}, and  collaboration due to indirect reciprocity, relying on social capital inherent in closed triads \cite{righi2018social}) since units may be influenced by their neighboring units and by the network structure \cite{everett1990ego,pattison1993algebraic}.


\begin{figure}
    \centering
\begin{tikzpicture}
\begin{scope}[every node/.style={circle,thick,draw}]
    \node (A) at (2,3) {3};
    \node (B) at (0,3) {2};
    \node (C) at (1,4) {1};
    
    \node[fill=blue!25] (D) at (6,3) {6};
    \node (E) at (4,3) {5};
    \node[fill=blue!25] (F) at (5,4) {4};
    
    % \node[fill=ForestGreen] (G) at (6,0) {G};
    % \node[fill=ForestGreen] (H) at (4,0) {H};
    % \node[fill=ForestGreen] (I) at (5,1) {I};
    
    \node (J) at (3,2.7) {8};
    \node (K) at (4,1.8) {10};
    \node (L) at (1,2) {7};
    \node (M) at (2,1.3) {9};
\end{scope}

\begin{scope}[>={Stealth[black]},
            %   every node/.style={fill=white,circle},
              every edge/.style={draw=red,very thick}]
    \path [-] (A) edge node {} (B);
    \path [-] (A) edge node {} (C);
    \path [-] (B) edge node {} (C);
    
    \path [-] (D) edge node {} (E);
    \path [-] (D) edge node {} (F);
    \path [-] (E) edge node {} (F);
    
    % \path [-] (G) edge node {} (H);
    % \path [-] (G) edge node {} (I);
    % \path [-] (H) edge node {} (I);
    
    % \path [-] (A) edge node {} (J);
    % \path [-] (E) edge node {} (J);
    % \path [-] (I) edge node {} (K);
    % \path [-] (J) edge node {} (K);
    % \path [-] (L) edge node {} (B);
    % \path [-] (H) edge node {} (M);
    % \path [-] (M) edge node {} (L);
    % \path [-] (D) edge node {} (G);
    
    \path [-] (L) edge node {} (J);
    \path [-] (K) edge node {} (M);
    
\end{scope}
\end{tikzpicture}
    \caption{Network of social contacts corresponding to the units in Table \ref{tbl:covariates}. Blue nodes are positively affected by the treatment}\label{fig:socialnet}
\end{figure}

\begin{table}[h]
    \centering \footnotesize
    \caption{ Table of the units in the social network shown in Figure \ref{fig:socialnet}. The gray column shows the effect of being in an SHG on having outstanding loans and the blue units are positively affected by the treatment}\label{tbl:covariates}
  \begin{tabular}{ccccc||a}
    \toprule
     ID &  Occupation ($O$) &  Election Card ($E$) &  SHG ($T$) &  Loan ($Y$) & TE \\ %$X_{:,1}$, $X_{:,2}$
    \hline
    1 &           Farm Labour &              Yes &        Yes &     No & 0 \\
    2 &           Factory worker &              No &     No &     Yes & 0.5  \\
    3 &           Farm Labour &              Yes &        Yes &     No & 0\\
    \rowcolor{blue!25}
    4 &           Farm Labour &                No &      Yes &     Yes & 1 \\
    5 &           Farm Labour &              Yes &        Yes &     Yes & 0.5 \\
    \rowcolor{blue!25}
    6 &           Farm Labour &              No &        No &     No & 1 \\
    7 &           Farm Labour &           Yes &        Yes &     Yes & 0 \\
    8 &           Factory worker &              Yes &    Yes &     Yes & 0 \\
    9 &           Factory worker &              No &    No &     Yes & 0 \\
    10 &           Factory worker &             No &    Yes &     Yes & 0\\
    \bottomrule
    \end{tabular}
   
    \vspace{-3mm}
\end{table}


% \babak{I subject merging both examples, the example needs to explain the heterogeneity and effect modifiers and why its challenging to discover them in social networks}
\begin{example}\label{ex:hyp_intro}
In developing countries like India, it is challenging for many poor households to have access to financial instruments such as loans and insurance plans due to lack of assets, monetary support, or knowledge. Inability to access these financial instruments often impedes the entrepreneurial growth of micro and small-scale farmers and businesses. In this situation, self-help groups (SHG) or saving groups have become quite popular across villages in India and are also promoted by the government. The concept of SHG is primarily rooted in the idea to create a larger pool of monetary asset with relatively small scale participation to pool the financial risk. 
Often, individuals who are part of an SHG can use the pooled wealth as mortgage for loans. 
% We are therefore interested in examining the causal effect of self-help groups (SHG) on financial risk tolerance using 2010 survey data from 77 villages in Karnataka, India \cite{jackson2012social,banerjee2014gossip,microfinancedata}.
We use a 2010 survey data from 77 villages in Karnataka, India \cite{jackson2012social,banerjee2014gossip,microfinancedata} to examine the causal effect of belonging to an SHG on financial risk tolerance (measured as the presence of outstanding loans).
% , using 2010 survey data from 77 villages in Karnataka, India \cite{jackson2012social,banerjee2014gossip,microfinancedata}. 
The survey contains data about individuals in two forms: their social interactions with non-relatives (a toy example of the social network is shown Figure \ref{fig:socialnet}), along with information about each person (shown in Table \ref{tbl:covariates}). 
The information displayed in Table \ref{tbl:covariates} includes, for each person, the occupation of that person, whether they have an election card (an identity proof for Indian citizens), whether they have savings, whether they belong to an SHG, and whether they have outstanding loans. 
A causal inference algorithm can then estimate for each person, the effect of being in an SHG on having outstanding loans. This treatment effect is shown in the gray column in Table \ref{tbl:covariates}. 
\amir{do we still need to color some of the units blue?}
% where the units whose rows are colored blue have been positively affected by being in an SHG. 

Notice that there are three distinct values in the gray column, namely $0, 0.5$, and $1$, thus, there is heterogeneity in the treatment effect. 
% Consider persons $1$ and $4$. The treatment effect of person $1$ is $0$ while the treatment effect of person $4$ is $1$, thus, there is heterogeneity in the treatment effect. 
Furthermore, consider the Election Card column. All people with election cards have treatment effect $\leq 0.5$ (in particular, there are those with treatment effect $0$), while all people without them have treatment effect $\geq 0.5$  (in particular, there are those with treatment effect $1$). Thus, splitting the population into two groups: those with an election card and those without it will split the treatment effect as well. Thus, election card is an effect modifier. 

Suppose we are further interested in testing whether two other properties are effect modifiers: (1) interactions with people who work in Farm Labour and (2) being part of a triad (i.e., belong to a 3-clique). 
This requires analysis that goes beyond knowing the properties of each person, given in Table \ref{tbl:covariates}, 
% since we also have to know the information about their neighbors in the social network, the effect of the neighbors on each person, and the effect of the local network structure on each person. 
since we also have to consider the treatment effect of the neighbors of each person, and the effect of the local network structure on a person. 
\end{example}
% \begin{example}\label{ex:hyp_intro}
% Once the treatment effect has been estimated, 
% we are further interested in testing the following hypothesis about the data: are people who (1) have an election card, (2) who have interactions with people who work in Farm Labour and (3) are part of a triad (i.e., belong to a 3-clique), more likely to benefit from participating in an SHG?, i.e., are they more likely to not have an outstanding loan if they belongs to an SHG? 
% To test this hypothesis we need to consider three factors: the information of an individual, the information about their neighbors in the social network, and the network structure.
% \end{example}


% The researchers performing causal inference may further be interested in {\em understanding which covariates played a role in influencing the treatment effect}, or, formally, which covariates are effect modifiers \cite{hernan2010causal,vanderweele2007four}. 
% If the treatment effect changes across populations with different values of a covariate, this covariate is called an effect modifier. 
%The researchers performing causal inference may further be interested in understanding {\em how different groups in the population responded to the treatment}, or, formally, which covariates are effect modifiers \cite{hernan2010causal,vanderweele2007four}. Finding such effect modifiers can assist researchers to understand how to plan a policy (e.g., a vaccine rollout policy may change when knowing that children under $10$ are less affected by the vaccine), and, in general, identifying the factors that influence the outcome, which may become another form of treatment (e.g., in a vaccine efficacy trial, if people who do regular physical exercise are more benefited by the vaccine, researchers can then try to investigate the relation between the vaccine effect and physical exercise). 

We propose a novel framework for the estimation of treatment effect heterogeneity and detecting effect modifiers, tailored to causal inference in social networks. 
%  First, we formalize complex effect modifiers that may arise because of complex social interaction between the subjects, i.e., effect modifiers associated with the neighbors' covariates on the outcome and the network structure associated with each subject. 
First, we define a causal model for social networks that captures complex effect modifiers that may arise because of complex social interaction between the subjects, i.e., effect modifiers associated with the neighbors' covariates on the outcome and the network structure associated with each subject. 
% Second, we propose a novel hypothesis testing approach to  .... .   \babak{Flesh out the contributions here}
Second, we propose a novel hypothesis testing approach based on the standard $I^2$ test \cite{higgins2003measuring} that accounts for neighbors' covariates and patterns in the social network. 
Third, we provide an algorithm for testing effect modifiers. The algorithm relies on ideas from graph theory to handle network patterns \cite{houbraken2014index} and ideas from relational causal inference to handle neighbors' covariates \cite{DSalimiPKGRS20}. 
Finally, we perform experiments using both synthetic data (simulating a vaccine trial) and real data (the network demonstrated in our example), showing the our solution is able to detect the true effect modifiers and is relatively insensitive to high levels of noise. 
 
 \babak{Here brag about the importance of the analytics provided by your system} 
Using our framework researchers can create and test hypotheses about complex effect modifiers in terms of network features or network patterns. 
For example, whether agents might financially cooperate due to indirect reciprocity relying on social capital inherent \cite{righi2018social}. 
The analysis provided by our framework plays a critical role in (1) testing for the existence or lack of heterogeneous treatment effects, (2) identifying sub-populations
for which a treatment is effective or harmful, (3) generalizing causal effect estimates obtained from a study sample to a target population. 
 
%Moreover, effect modifiers can assist researchers in learning about the transportability of the treatment across different population \cite{pearl2014external,hernan2010causal}, i.e., the ability to extrapolate causal effects computed in one population to another population.  Since the data collected comprises a social network, the effect modifiers can refer to the features of each unit, the features of its neighbors in the network, and the local structure of the network surrounding each unit. 


% \babak{Move the following to related work} A large body of work has been dedicated to devising ways to test statistical hypotheses (e.g., \cite{snyder1978hypothesis,xia2017hypothesis,LAROSA201581,shaffer1995multiple,list2019multiple,viechtbauer2007hypothesis}). In particular, previous work has proposed hypotheses tests for the heterogeneity of a population in a study \cite{viechtbauer2007hypothesis}. These include heterogeneity tests such as Cochran's Q \cite{cochran1954combination}, $H$ statistics, $R$ statistics, and $I^2$ \cite{higgins2002quantifying,higgins2003measuring}. 
% However, such tests are limited to discrete covariates and they do not take into account the context of the social network, i.e., the possible effect of the neighbors' covariates on the outcome and the network structure associated with each unit. In the context of our running example, existing tests cannot examine whether neighbors occupation and belonging to a 3-clique are effect modifiers. 

%{\em In this paper we propose a novel test for treatment effect modifiers tailored to causal inference in social networks}. 
\babak{I stopped here}
Next overview our contributions in more detail. 


\paratitle{Model and test:} Our criterion for testing possible effect modifiers is based on $I^2$ \cite{higgins2003measuring} but allows for 
% (1) continuous covariates, 
(1) graph patterns and (2) summarized neighbors' covariates. 
% For (1), we define our test using an integral over the covariate values. This models the test more accurately than the standard sum over the values. 
For (1), we define a desideratum for matching graph patterns to the subgraphs that include each unit in the social network. Intuitively, we define a graph pattern with a specific distinguished node and say that a graph pattern matches a subgraph of a unit if there is a subgraph isomorphism from the pattern to the subgraph where the distinguished node is mapped to the unit. 
For (2), since the number of neighbors of each unit in the network may be different, we build on the notions of covariate summary proposed in previous work \cite{DSalimiPKGRS20}. Given a covariate of a unit in the social network, we aggregate this covariate across all neighbors into a single summarized number (e.g., the percentage of neighbors who work as Farm Labour). 

\paratitle{Algorithms for testing:} We devise an algorithmic solution for testing hypothesized effect modifiers according to our criterion. The algorithms incorporate ideas from causal inference, hypothesis testing and graph theory. Namely, our solution uses causal inference to compute the treatment effect for each unit (conditional treatment effect) and subgraph isomorphism concepts (using the ISMAGS algorithm \cite{houbraken2014index}) to compute the value of the hypothesized effect modifier for each unit. 
Once these are computed, our solution estimates the influence of the covariate on the treatment effect using regression. 

\paratitle{Experimental study:} We provide an extensive experimental evaluation using a real social network based on a 2010 survey data from 77 villages in Karnataka, India \cite{jackson2012social,banerjee2014gossip,microfinancedata} (our running example) as well as synthetic data, simulating a vaccine efficacy trial. 
Through the synthetic data, we examine the effect of the number of units and the noise in the potential outcome on our test. 
Our results indicate that as the number of units increases (up to $4096$), the real effect modifiers
Through the real data, we demonstrate a use-case, showing our system's performance and its ability to find effect modifiers in a large scale network ($\sim$ 17K units). 

% In statistical studies, researchers often require tools for testing their hypotheses in an efficient and reliable manner.
% Hypothesis testing is therefore an important cornerstone in statistics and it has been studied in various settings and contexts (e.g., \cite{snyder1978hypothesis,xia2017hypothesis,LAROSA201581,shaffer1995multiple,list2019multiple}). There are multiple ways of testing hypotheses 
 

==> multiple.tex <==
\subsection{Generating the Hypothesized Matrix}
\amir{add text}


\begin{table}[h]
    \centering \footnotesize
    \caption{\amir{verify:}Hypothesized matrix for the hypothesis in Example \ref{ex:hypothesis}. $X_i$ is the indicator for possessing as election card, $N_i$ is the portion of neighbors who work as Farm Labour, and $G_i$ is the indicator for an existence of a pattern-preserving isomorphism from a 3-clique to the ego-centrix graph of $i$}\label{tbl:hypothesis_matrix}
  \begin{tabular}{|c|c|c|c|c}
    % \toprule
    \hline
    \rowcolor{Gray}
     ID &  $X_i$ &  $N_i$ &  $G_i$ \\
    \hline
    % has election card, neighbors' percentage with occupation farm, is in triangle
    1 & 1 & 0.5 & 1\\
    \hline 2 & 0 & 1 & 1\\
    \hline 3 & 1 & 0.5 & 1\\
    \hline 4 & 0 & 1 & 1\\
    \hline 5 & 1 & 1 & 1\\
    \hline 6 & 0 & 1 & 1\\
    \hline 7 & 1 & 0 & 0\\
    \hline 8 & 1 & 1 & 0\\
    \hline 9 & 0 & 0 & 0\\
    \hline 10 & 0 & 0 & 0\\
    % \bottomrule
    \hline
    \end{tabular}
\end{table}


\begin{definition}[Hypothesized Matrix]
Given a social network $G = (V,E)$ and a hypothesized covariate vector $h$, a hypothesized matrix $U$ is a matrix where the $i$'th row is the realized values of the hypothesized covariates of $h$ to hypothesized covariate vector for unit $i \in V$.
\end{definition}

\begin{example}
Table \ref{tbl:hypothesis_matrix} depicts the hypothesized matrix for the hypothesis in Example \ref{ex:hypothesis}. For example, in the first row, for unit $1$ we have that $X_1 = 1$, i.e., this unit has an election card, $N_i = 0.5$, i.e., 1 out of 2 neighbors work as Farm Labour and $G_1 = 1$, i.e., there is a pattern-preserving isomorphism from a 3-clique to the ego-centric graph of $i$.
\end{example}


\begin{algorithm}[!htb]
	\SetKwFunction{Generate Hypothesized Matrix}{Generate Hypothesized Matrix}
	\SetKwInOut{Input}{input}\SetKwInOut{Output}{output}
	\LinesNumbered
	\SetKwProg{enhance}{$\texttt{genHypMatrix}$:}{}{}
	\Input{Table of units covariates $U$, hypothesized covariate vector $h = (X,N,P)$,
% 	node list of a node in each pattern in $g$ $\mathcal{U}$, 
% 	a list of metric vectors for the covariates of the nodes in the patterns $\mathcal{M}$, a list of threshold vectors for the covariates $\mathcal{T}$
    }
    \Output{A hypothesized matrix $U_h$}
	\BlankLine
	\enhance{}{
	$U_h \gets EmptyMatrix()$\;
    \ForEach{$i \in U$}
	    {\label{l:iterate_nodes}
	        \ForEach{$c \in X$}
	        {\label{l:iterate_covar}
	            $U_h[i].append(U[i][c])$\;
    	    }
	        \ForEach{$c \in N$}
	        {\label{l:iterate_covar}
	            $U_h[i].append(embed(\{U[j][c] ~|~ j\in N(i)\}))$\;
    	    }
    	    \ForEach{$p \in P$}
	        {\label{l:iterate_patterns}
	            $isPatt \gets \texttt{checkGraphPattern}(G[N(i)],p,i)$\;
	           % $isExp \gets \texttt{checkExpPattern}(G[N(i)],p,i,u,\mathcal{M}[j],\mathcal{T}[j])$\;
	            $U_h[i].append(isPatt)$\;
	        }
	    }
	\Return $U_h$\;
	}
	\caption{Generate Hypothesized Matrix}
	\label{algo:enhance_table}
\end{algorithm}


\begin{algorithm}[!htb]
	\SetKwFunction{Monte Carlo Sampling}{Monte Carlo Sampling}
	\SetKwInOut{Input}{input}\SetKwInOut{Output}{output}
	\LinesNumbered
	\Input{Social network $\mathbf{G}$, unit table $\mathbf{U}$, causal graph $\mathcal{G}$ hypothesized covariate vector $h$, 
% 	a node in $P$ $u$, a metric vector for the covariates $\vec{m_c}$, 
% 	a threshold vector for the covariates $\vec{\tau_c}$,
	number of repeats $m$, sample size $k$}
    \Output{Contribution of $h$ to heterogeneity}
	\BlankLine
% 	$Q \gets [[]]$\;
% 	\For {$1 \text{ to } m$}
	\label{l:iterate_sample}
        % $U_s \leftarrow \texttt{sampleSubset}(U, s)$\;\label{l:sample}
        $CDE \gets \texttt{causalInference}(\mathbf{U},\mathbf{G},\mathcal{G})$\;
        $ADE \gets mean(CDE)$\;
        
        $U^h \gets \texttt{genHypMatrix}(\mathbf{U},\mathbf{G},h)$\;
        %  $g \gets project(CDE, U^h)$\;
        $q \gets []$\;
        \ForEach{$1\leq j \leq |h|$}
       {
            $g \gets project(CDE, U^h_{:,j})$\;
            $\{ u_{i,j} \}_{i=1}^k \widesim{i.i.d} Uniform(Dom(U^h_{:,j}))$\;
            $q_j \gets 
            % \frac{\partial g(U_h)}{\partial U_h.j}$\;
            \sum_{u_{i,j}}\frac{\left(mean(g(u_{i,j})) - ADE\right)^2}{\widehat{var}(g(u_{i,j}))}$;
            % $accum[j] \gets \int_{U_h.j} deriv$\;
       }
       $I^2 \gets \left[100\cdot \frac{q_j - k + 1}{q_j}\right]_{j=1}^{|h|} $\;
	\Return $I^2$\;
	\caption{Test Hypothesis}
	\label{algo:monte_carlo_sampling}
\end{algorithm}

\begin{example}\label{ex:monte_carlo_sampling}
\amir{update}
Reconsider our running example. 
We demonstrate Algorithm \ref{algo:monte_carlo_sampling} where the input is the social network graph $G$ shown in Figure \ref{fig:socialnet}, the 3-clique pattern with the same covariates as for unit $C$ as $P$, $C$ as node $i$, any node in $P$ as $u$, $\vec{m_c} = (|\cdot|, |\cdot|, |\cdot|)$, and $\vec{\tau_c} = (0, 0, 0)$, $m=2$, $s=1$. 
The algorithm initializes $\varphi$ to $0$ and then performs a single iteration. Suppose that in line \ref{l:sample} the algorithm samples the node $C$. In line \ref{l:node_contribute}, Algorithm \ref{algo:check_explanation_pattern} will return True as we show in Example \ref{ex:check_explanation_pattern} and we also know that $CDE(C) = 1$ as we have seen in Example \ref{ex:cde}. Thus, in line \ref{l:increment_varphi1}, the algorithm updates $\varphi_1$ to $1$. Then, in lines \ref{l:mean_diff}-\ref{l:hetero_add} the algorithm updates $h = 1$ and adds $1$ to the list $Heterogeneity$. 
Now suppose that in the second iteration, $L$ is sampled. In line \ref{l:node_contribute}, Algorithm \ref{algo:check_explanation_pattern} will return False (a subgraph of $G[N(L)]$ is not isomoprphic to a 3-clique). It holds that $CDE(L) = -1$, so in line \ref{l:increment_varphi1}, the algorithm updates $\varphi_0$ to $-1$. 
In lines \ref{l:mean_diff}-\ref{l:hetero_add} the algorithm updates $h = 1$ and adds $1$ to the list $Heterogeneity$. 
After exiting the loop in line \ref{l:iterate_sample}, the algorithm computes and returns $z = 1$, which is computed in line \ref{l:no_std} (since the std is $0$). 
\end{example}

\blue{SR: After everything else is stable for single-covariate hyp testing (no conditioning) including background, prelim, algos, and experiments, we can come back to conditional hypothesis testing (conditioning on everything else in $h$) that would require going through the causal DAG and concrete definitions, possibly also monotonicity proofs/counterexamples -- e.g., if A is an effect modifier, A conditioned on B, C is not, then is A|B effect modifier (or vice versa). The age is an effect modifier but age|edu is not as much is a good example.}

\amir{To confound Type I and Type II error, prove:}Define the error as the L1 distance between the actual value $\hat{z}$ computed over the entire unit table and the value returned by Algorithm \ref{algo:monte_carlo_sampling}, denoted by $z$. We next prove that $|\hat{z} - z| \to 0$ as $m \to \infty$ and $s \to \infty$.

==> old/intro-827pm-saved.tex <==
abstract:

We study {\em treatment effect modifiers} for causal analysis in a social network, where neighbors' characteristics or neighborhood structure may affect the outcome of a unit, and the goal is to identify sub-populations with varying treatment effects using such network properties. We propose a novel framework called \emph{Testing-for-Effect-Modifier (TEEM)} for this purpose that facilitates data-driven decision making by testing hypotheses about complex effect modifiers in terms of network features or network patterns  (e.g., characteristics of neighbors of a unit or belonging to a triangle), and by identifying sub-populations for which a treatment is likely to be effective or harmful. We describe a hypothesis testing approach that accounts for unit's covariates, their neighbors' covariates and patterns in the social network, and devise an algorithm incorporating ideas from causal inference, hypothesis testing, and graph theory to verify a hypothesized effect modifier. We perform  extensive experimental evaluations with a real development economics dataset about the treatment effect of belonging to a financial support network called self-help groups on risk tolerance, and also with a synthetic dataset with known ground truths simulating a vaccine efficacy trial, to evaluate our framework and algorithms.  





\section{introduction}\label{sec:intro}
%\amir{Intro on causal inference. Needs to be expanded:}



Causal inference is at the heart of empirical research and principled decision-making in natural and social sciences, and is practically indispensable in epidemiology \cite{robins2000marginal}, clinical research \cite{clinicaltrials2007}, 
public policy \cite{manski2013public}, economics \cite{banerjee2011poor}, and other domains \cite{angrist1996identification,angrist2008mostly}. In causal inference, we go beyond establishing correlation or prediction, and are interested in making causal statements using the concepts of \emph{counterfactuals} and \emph{interventions} about a \emph{treatment} (e.g., administering a vaccine) on some \emph{outcome} of interest (e.g., not being infected by the targeted disease). While a \emph{randomized controlled trial}, which divides the participating \emph{units or subjects} into \emph{treatment and control groups} at random and evaluates the difference of outcome in these two groups, is considered the gold standard for causal analysis, due to cost or ethics concerns, we often need to rely on \emph{observational causal studies} %in data science 
using collected data under various assumptions as studied in the literature in statistics (e.g., Rubin's potential outcome framework \cite{Rubin1974}) or AI (e.g., Pearl's probabilistic causal model \cite{pearl2000book}).    
%\red{update last line}.
%\red{another sentence/Rubin-Pearl}
\par
A typical assumption made in the causality literature is {\em no-interference} or \emph{independence} among units, %\cite{Rubin1974} \red{correct cite?}, 
meaning that the assigned treatment %or the outcome 
of one unit should \emph{not} affect the outcome of another unit (called \emph{interference or spill-over effects})
%and \emph{contagion} respectively)
\cite{ogburn2017causal, DSalimiPKGRS20}
%\red{cite}
%which requires the unit of a study not to have causal interaction with other units through ,~
\footnote{Rubin’s potential outcome framework \cite{Rubin1974}, which is a prominent approach for causal inference in statistical studies, relies on the ``\emph{Stable Unit Treatment Value Assumption (SUTVA)}'', which includes the assumption of no-interference.}.
%meaning that treating one unit should not causally influence the outcome of others. 
However, in many studies in social science, the units may directly or indirectly interact with each other in different ways and as a result, a unit's outcome %(behaviour or states) 
might be influenced by the %treatment
behavior, states, or characteristics of its social ties in a network, which leads to violation of the no-interference assumption \cite{VanderWeele-book-2013}. 
%\babak{reword the following examples, use examples from social science or add other disciples the the previous sentences} \amir{add one more here}
Examples of such interference include detecting evidence of indirect protection from cholera vaccines when the vaccination rate of individuals in the social network is high \cite{root2011role},
% determining the effect of fake news spreading on elections \cite{bovet2019influence},
or showing that indirect reciprocity inherent in closed triads is linked to cooperation between individuals \cite{righi2018social}. 
% since units may be influenced by their neighboring units and by the network structure \cite{everett1990ego,pattison1993algebraic}.
%%%%%%SR -- useful: https://cdn1.sph.harvard.edu/wp-content/uploads/sites/603/2020/07/SNChapter_Book.pdf


This paper focuses on the study of {\em treatment effect modifiers~\cite{pearl2017detecting} or effect heterogeneity for causal analysis in a social network}. In a causal study, different units may exhibit different levels of response to the applied treatment based on their characteristics, and the effect heterogeneity problem aims to infer this degree %which the applied treatment has different 
of causal effects on different units. As an example, one of the key objectives in clinical research is not only to discover effects of %social programs or 
medical treatments at the entire population-level, but also to ascertain 
%{\em treatment effect modifiers} or 
treatment effects on 
different sub-populations (e.g., whether a new vaccine is beneficial or harmful based on age or previous health conditions of individuals).
%is beneficial or harmful. For instance, in medical trials, the goal is to identify sub-populations  for which a treatment  ~\cite{brinkley2010generalized}.  
While different hypothesis tests for the heterogeneity of a population in a study have been proposed in the literature \cite{viechtbauer2007hypothesis, athey2016recursive}, along with a large body of work on testing statistical hypotheses (e.g., \cite{snyder1978hypothesis,xia2017hypothesis,LAROSA201581,shaffer1995multiple,list2019multiple}), such tests 
%are limited to discrete covariates of units and 
do not take into account the context of the social network like possible effects of the neighbors' covariates or the network structure on the outcome. On the other hand, while there has been a recent surge of interest in causal inference in social networks~\cite{ogburn2017causal,ogburn2018causal,awan2020almost, DBLP:conf/uai/ShermanS19}, they have not focused on the effect heterogeneity problem. Indeed, reasoning about effect modification and heterogeneity in social networks %is a %very challenging problem. 
poses new conceptual and computational challenges. We illustrate a possible scenario in the following example.   
%i.e., the possible effect of the neighbors' covariates on the outcome and the network structure associated with each unit.

%\sudeepa{Edited up to here.}

\cut{
Recently, , as well as to a lesser extent, 
%Much of 
this literature, however, has not addressed the problem of {\em effect heterogeneity}, defined as the degree which different treatments have different causal effects on each unit~\cite{..} \red{cite}. Much literature has focused on detecting heterogeneity and effect modifiers, however, not in the presence of interference and social networks \cite{athey2016recursive}. 
}





\begin{table}[t]
    \centering \footnotesize
    \caption{A toy table of units for Example~\ref{ex:hyp_intro}. 
    %in the social network shown in Figure \ref{fig:socialnet}. The gray column shows the treatment effect (TE) of being in an SHG on having outstanding loans.
    %and the blue units are positively affected by the treatment
    }\label{tbl:covariates}
  \begin{tabular}{ccccc||a}
    \toprule
     ID &  Occupation ($O$) &  Election Card ($E$) &  SHG ($T$) &  Loan ($Y$) & TE \\ %$X_{:,1}$, $X_{:,2}$
    \hline
    1 &           Farm Labour &              Yes &        Yes &     No & 0 \\
    2 &           Factory worker &              No &     No &     Yes & 0.5  \\
    3 &           Farm Labour &              Yes &        Yes &     No & 0\\
   % \rowcolor{blue!25}
    4 &           Farm Labour &                No &      Yes &     Yes & 1 \\
    5 &           Farm Labour &              Yes &        Yes &     Yes & 0.5 \\
   % \rowcolor{blue!25}
    6 &           Farm Labour &              No &        No &     No & 1 \\
    7 &           Farm Labour &           Yes &        Yes &     Yes & 0 \\
    8 &           Factory worker &              Yes &    Yes &     Yes & 0 \\
    9 &           Factory worker &              No &    No &     Yes & 0 \\
    10 &           Factory worker &             No &    Yes &     Yes & 0\\
    \bottomrule
    \end{tabular}
   
    \vspace{-3mm}
\end{table}


% \babak{I unit merging both examples, the example needs to explain the heterogeneity and effect modifiers and why its challenging to discover them in social networks}
\begin{example}\label{ex:hyp_intro}
In developing countries like India, it is challenging for many poor households to have access to financial instruments such as loans and insurance plans due to lack of assets, monetary support, or the necessary knowledge. 
% Inability to access these financial instruments often impedes the entrepreneurial growth of micro and small-scale farmers and businesses. 
In this situation, self-help groups (SHG) or saving groups have become quite popular across villages in India and are also promoted by the government. 
A SHG \cite{nailaSHG2005} is a voluntary community-based group with a small number of members  (typically 10-20, and often comprising women from similar social and economic backgrounds), %to save small sums of money, on a regular basis. They 
who pool their resources to become financially stable, taking loans from their collective savings in times of emergency, important life events, or to purchase assets.
%The idea behind SHG is to create a larger pool of monetary assets with relatively small scale participation to pool the financial risk. 
Often, individuals who are part of an SHG can use the pooled wealth as mortgage for loans. 
We use a 2010 survey data from 77 villages in Karnataka, India \cite{jackson2012social,banerjee2014gossip,microfinancedata} to examine the causal effect of belonging to an SHG on financial risk tolerance (measured as the presence of outstanding loans).
The survey contains data about individuals in two forms: their social interactions with non-relatives (a toy example of the social network is shown in Figure \ref{fig:socialnet}), along with information about each person (shown in Table \ref{tbl:covariates}). 
The information displayed 
%covariates collected 
for each person in Table \ref{tbl:covariates} includes the occupation of that person, whether they have an election card (an identity proof for Indian citizens), whether they have savings, whether they belong to an SHG, and whether they have outstanding loans. 
A causal inference algorithm can then estimate for each person, the effect of being in an SHG (treatment) on having outstanding loans (outcome). This estimated \emph{treatment effect (TE)} is shown in the gray column in Table \ref{tbl:covariates} that we formally define in Section~\ref{sec:background}. 
%\amir{do we still need to color some of the units blue?}
% where the units whose rows are colored blue have been positively affected by being in an SHG. 

Notice that there are three distinct values in the gray column, namely $0, 0.5$, and $1$, thus, there is heterogeneity in the treatment effect. 
% Consider persons $1$ and $4$. The treatment effect of person $1$ is $0$ while the treatment effect of person $4$ is $1$, thus, there is heterogeneity in the treatment effect. 
Furthermore, consider the Election Card (E) column. All people with election cards have treatment effect $\leq 0.5$ (in particular, there are those with treatment effect $0$), while all people without them have treatment effect $\geq 0.5$  (in particular, there are those with treatment effect $1$). Thus, splitting the population into two groups: those with an election card and those without it will split the treatment effect as well, suggesting election card is a potential effect modifier. 

Suppose we are further interested in testing whether two other properties are effect modifiers: (1) interactions with people who work in Farm Labour, and (2) being part of a triad (i.e., belong to a 3-clique). 
This requires analysis that goes beyond knowing the properties of each person given in Table \ref{tbl:covariates}
since we also have to consider the features of the neighbors as well as local network structure  of each person as shown in Figure~\ref{fig:socialnet}. 
%the treatment effect of the neighbors of each person, and the effect of the local network structure on a person. 
\end{example}
\begin{figure}[t]
    \centering
\begin{tikzpicture}[scale=0.7]
\begin{scope}[every node/.style={circle,thick,draw}]
    \node (A) at (2,3) {3};
    \node (B) at (0,3) {2};
    \node (C) at (1,4) {1};
    
    \node (D) at (6,3) {6};
    \node (E) at (4,3) {5};
    \node (F) at (5,4) {4};
    
    \node (J) at (3,2.7) {8};
    \node (K) at (4,1.8) {10};
    \node (L) at (1,2) {7};
    \node (M) at (2,1.3) {9};
\end{scope}

\begin{scope}[>={Stealth[black]},
            %   every node/.style={fill=white,circle},
              every edge/.style={draw=red,very thick}]
    \path [-] (A) edge node {} (B);
    \path [-] (A) edge node {} (C);
    \path [-] (B) edge node {} (C);
    
    \path [-] (D) edge node {} (E);
    \path [-] (D) edge node {} (F);
    \path [-] (E) edge node {} (F);
    
    \path [-] (L) edge node {} (J);
    \path [-] (K) edge node {} (M);
    
\end{scope}
\end{tikzpicture}
    \caption{An example network of social contacts corresponding to the units in Table~\ref{tbl:covariates} for Example~\ref{ex:hyp_intro}. 
    %Blue nodes are positively affected by the treatment
    }\label{fig:socialnet}
\end{figure}
\vspace{-0.4cm}
\subsection*{Our Contributions}
%\amir{This part consolidates the previous and current versions}
We propose a novel framework called \textbf{ Testing-for-Effect-Modifier (TEEM)} for the estimation of treatment effect heterogeneity and detecting effect modifiers, tailored to causal inference in social networks. 
With our framework, researchers can create and test hypotheses about complex effect modifiers in terms of network features or network patterns, e.g., 
%For example, 
whether agents might financially cooperate due to indirect reciprocity relying on social capital %inherent 
\cite{righi2018social}. 
The %analysis provided by our 
TEEM framework facilitates decision makings and effective interventions by allowing
%plays a critical role in %(1) 
\begin{enumerate}
\itemsep0em
    \item testing for existence or lack of existence for various kinds of heterogeneous treatment effects using summarized properties of network features or neighborhood structures,
    \item  identification of sub-populations
for which a treatment is effective, neutral, or harmful, and
\item generalization of causal effect estimates and causal conclusions obtained from a study sample to a target population based on relative distributions of different sub-populations. 
\end{enumerate}
Our technical contributions in the paper are as follows.
%, (2), (3) 

%We next overview our contributions in detail:
\noindent
\textbf{Model and framework:} 
We define a causal model for social networks that captures complex effect modifiers that may arise because of complex social interaction between the units, i.e., effect modifiers associated with the neighbors' covariates on the outcome and the network structure associated with each unit. 
We then propose a novel hypothesis testing approach based on the standard $I^2$ test \cite{higgins2003measuring} that accounts for neighbors' covariates and patterns in the social network.
Since the number of neighbors of each unit in the network may be different, we use the concept of covariate summary proposed in %previous work 
\cite{DSalimiPKGRS20}. Given a covariate of a unit in the social network, we aggregate this covariate across all neighbors into a single summarized number (e.g., the percentage of neighbors who work as Farm Labour). We further define a desideratum for matching network patterns to parts of the social network. Intuitively, we define a network pattern with a specific distinguished node and say that a network pattern matches the local network structure of a unit if there is a subgraph isomorphism from the pattern to the subgraph where the distinguished node is mapped to the unit. 

\paratitle{Algorithm for testing:} 
We devise an algorithm for testing effect modifiers. 
The algorithms incorporate ideas from causal inference, hypothesis testing, and graph theory. In particular, our solution uses existing causal inference techniques from the literature to compute the treatment effect for each unit (conditional treatment effect) and subgraph isomorphism concepts to compute the value of the hypothesized effect modifier for each unit. 
Once these are computed, our solution estimates the influence of the covariate on the treatment effect. 

\paratitle{Experimental study:} We provide an extensive experimental evaluation using the real social network described in our example \cite{jackson2012social,banerjee2014gossip,microfinancedata} as well as synthetic data with known ground truth simulating a vaccine efficacy trial. 
Through the synthetic data, we examine the effect of the number of units and the noise in the potential outcome on our test. 
Our results indicate that as the number of units increases, 
%(up to $4096$), 
the true effect modifiers become more evident and that our solution becomes relatively insensitive to high levels of noise. 
Through the real data, we demonstrate a use-case, showing our system's performance and its ability to find effect modifiers in a large scale network ($\sim$17K units).\\

\smallskip
\textbf{Roadmap.~} In the rest of the paper, we review some background concepts  (Section~\ref{sec:background}), describe our TEEM framework (Section~\ref{sec:model}), give algorithms (Section~\ref{sec:single}), describe the experimental study (Section~\ref{sec:experiments}), review related work (Section~\ref{sec:related}), and conclude with future research directions (Section~\ref{sec:conclusions}).



 

==> old/intro-after-SR-edited-first-two-para.tex <==
\section{introduction}\label{sec:intro}
%\amir{Intro on causal inference. Needs to be expanded:}



Causal inference is at the heart of empirical research and principled decision-making in natural and social sciences, and is practically indispensable in epidemiology \cite{robins2000marginal}, clinical research \cite{clinicaltrials2007}, 
public policy \cite{manski2013public}, economics \cite{banerjee2011poor}, and other domains \cite{angrist1996identification,angrist2008mostly}. In causal inference, we go beyond establishing correlation or prediction, and are interested in making causal statements using the concepts of \emph{counterfactuals} and \emph{interventions} about a \emph{treatment} (e.g., administering a vaccine) on some outcome of interest (e.g., not being infected by the targeted disease). While a \emph{randomized controlled trial}, which randomly divides the participating \emph{subjects or units} into \emph{treatment and control groups} at random and evaluates the difference of outcome in these two groups, is considered the gold standard for causal analysis, due to cost or ethics concerns, we often need to rely on \emph{observational causal studies} in data science using collected data under various assumptions as studied in the literature in statistics (e.g., Rubin's potential outcome framework \cite{Rubin1974}) or AI (e.g., Pearl's graphical causal model \cite{pearl2000book}).    
%\red{update last line}.
%\red{another sentence/Rubin-Pearl}
\par
A typical assumption made in the causality literature is {\em no-interference} or \emph{independence} among subjects, %\cite{Rubin1974} \red{correct cite?}, 
meaning that the assigned treatment or the outcome of one subject should \emph{not} affect the outcome of another subject (called \emph{interference} and \emph{contagion} respectively) \red{cite}
%which requires the subject of a study not to have causal interaction with other subjects through ,~
\footnote{Rubin’s potential outcome framework \cite{Rubin1974}, which is a prominent approach for causal inference in statistical studies, relies on the ``\emph{Stable Unit Treatment Value Assumption (SUTVA)}'', which includes the assumption of no-interference.}.
%meaning that treating one subject should not causally influence the outcome of others. 
However, in many studies in social science, the subjects may directly or indirectly interact with each other in different ways and as a result, a subject's outcome (behaviour or states) might be influenced by the %treatment
behavior, states, or characteristics of its social ties in a network, which leads to violation of the no-interference assumption \cite{VanderWeele-book-2013}. 
%\babak{reword the following examples, use examples from social science or add other disciples the the previous sentences} \amir{add one more here}
Examples of such interference include detecting evidence of indirect protection from cholera vaccines when the vaccination rate of individuals in the social network is high \cite{root2011role},
% determining the effect of fake news spreading on elections \cite{bovet2019influence},
or showing that indirect reciprocity inherent in closed triads is linked to cooperation between individuals \cite{righi2018social}. 
% since units may be influenced by their neighboring units and by the network structure \cite{everett1990ego,pattison1993algebraic}.
%%%%%%SR -- useful: https://cdn1.sph.harvard.edu/wp-content/uploads/sites/603/2020/07/SNChapter_Book.pdf


%This paper focuses on 
Recently, there has been a surge of interest in causal inference in social networks~\cite{ogburn2017causal,ogburn2018causal,awan2020almost, DBLP:conf/uai/ShermanS19}, as well as to a lesser extent, 
%Much of 
this literature, however, has not addressed the problem of {\em effect heterogeneity}, defined as the degree which different treatments have different causal effects on each subject~\cite{..} \red{cite}. The main objective in social and medial sciences is not to discover effect of social programs or medical treatments at population-level, but to ascertain {\em effect modifiers} or sub-populations across which the treatment effect differs. For instance, in medical trials, the goal is to identify subpopulations  for which a treatment is beneficial or harmful ~\cite{brinkley2010generalized}.  Much literature has focused on detecting heterogeneity and effect modifiers, however, not in the presence of interference and social networks \cite{athey2016recursive}. Indeed, reasoning about effect modification and heterogeneity social networks is a very challenging problem. We illustrate these challenges with the following example.  


%Causal inference exposes insights that are not always evident when using standard data science tools \cite{...}. Thus, it is the standard... 
%Standard causal inference is usually performed over units that can be represented as a single flat table, showing the traits of each unit. 
%\amir{Motivation for working with social networks:}


%However, in more complex realistic scenarios, social networks \cite{sailer1978structural,knoke2019social,wasserman1994social} may better describe additional attributes of the units, such as social relations and interactions \cite{valente2008correlated,granovetter1973strength}. These connections between units are useful in many studies (e.g., vaccine trials \cite{root2011role}, determining the effect of fake news spreading on elections \cite{bovet2019influence}, and  collaboration due to indirect reciprocity, relying on social capital inherent in closed triads \cite{righi2018social}) since units may be influenced by their neighboring units and by the network structure \cite{everett1990ego,pattison1993algebraic}.


\begin{figure}
    \centering
\begin{tikzpicture}
\begin{scope}[every node/.style={circle,thick,draw}]
    \node (A) at (2,3) {3};
    \node (B) at (0,3) {2};
    \node (C) at (1,4) {1};
    
    \node[fill=blue!25] (D) at (6,3) {6};
    \node (E) at (4,3) {5};
    \node[fill=blue!25] (F) at (5,4) {4};
    
    % \node[fill=ForestGreen] (G) at (6,0) {G};
    % \node[fill=ForestGreen] (H) at (4,0) {H};
    % \node[fill=ForestGreen] (I) at (5,1) {I};
    
    \node (J) at (3,2.7) {8};
    \node (K) at (4,1.8) {10};
    \node (L) at (1,2) {7};
    \node (M) at (2,1.3) {9};
\end{scope}

\begin{scope}[>={Stealth[black]},
            %   every node/.style={fill=white,circle},
              every edge/.style={draw=red,very thick}]
    \path [-] (A) edge node {} (B);
    \path [-] (A) edge node {} (C);
    \path [-] (B) edge node {} (C);
    
    \path [-] (D) edge node {} (E);
    \path [-] (D) edge node {} (F);
    \path [-] (E) edge node {} (F);
    
    % \path [-] (G) edge node {} (H);
    % \path [-] (G) edge node {} (I);
    % \path [-] (H) edge node {} (I);
    
    % \path [-] (A) edge node {} (J);
    % \path [-] (E) edge node {} (J);
    % \path [-] (I) edge node {} (K);
    % \path [-] (J) edge node {} (K);
    % \path [-] (L) edge node {} (B);
    % \path [-] (H) edge node {} (M);
    % \path [-] (M) edge node {} (L);
    % \path [-] (D) edge node {} (G);
    
    \path [-] (L) edge node {} (J);
    \path [-] (K) edge node {} (M);
    
\end{scope}
\end{tikzpicture}
    \caption{Network of social contacts corresponding to the units in Table \ref{tbl:covariates}. Blue nodes are positively affected by the treatment}\label{fig:socialnet}
\end{figure}

\begin{table}[h]
    \centering \footnotesize
    \caption{ Table of the units in the social network shown in Figure \ref{fig:socialnet}. The gray column shows the effect of being in an SHG on having outstanding loans and the blue units are positively affected by the treatment}\label{tbl:covariates}
  \begin{tabular}{ccccc||a}
    \toprule
     ID &  Occupation ($O$) &  Election Card ($E$) &  SHG ($T$) &  Loan ($Y$) & TE \\ %$X_{:,1}$, $X_{:,2}$
    \hline
    1 &           Farm Labour &              Yes &        Yes &     No & 0 \\
    2 &           Factory worker &              No &     No &     Yes & 0.5  \\
    3 &           Farm Labour &              Yes &        Yes &     No & 0\\
    \rowcolor{blue!25}
    4 &           Farm Labour &                No &      Yes &     Yes & 1 \\
    5 &           Farm Labour &              Yes &        Yes &     Yes & 0.5 \\
    \rowcolor{blue!25}
    6 &           Farm Labour &              No &        No &     No & 1 \\
    7 &           Farm Labour &           Yes &        Yes &     Yes & 0 \\
    8 &           Factory worker &              Yes &    Yes &     Yes & 0 \\
    9 &           Factory worker &              No &    No &     Yes & 0 \\
    10 &           Factory worker &             No &    Yes &     Yes & 0\\
    \bottomrule
    \end{tabular}
   
    \vspace{-3mm}
\end{table}


% \babak{I subject merging both examples, the example needs to explain the heterogeneity and effect modifiers and why its challenging to discover them in social networks}
\begin{example}\label{ex:hyp_intro}
In developing countries like India, it is challenging for many poor households to have access to financial instruments such as loans and insurance plans due to lack of assets, monetary support, or knowledge. Inability to access these financial instruments often impedes the entrepreneurial growth of micro and small-scale farmers and businesses. In this situation, self-help groups (SHG) or saving groups have become quite popular across villages in India and are also promoted by the government. The concept of SHG is primarily rooted in the idea to create a larger pool of monetary asset with relatively small scale participation to pool the financial risk. 
Often, individuals who are part of an SHG can use the pooled wealth as mortgage for loans. 
% We are therefore interested in examining the causal effect of self-help groups (SHG) on financial risk tolerance using 2010 survey data from 77 villages in Karnataka, India \cite{jackson2012social,banerjee2014gossip,microfinancedata}.
We use a 2010 survey data from 77 villages in Karnataka, India \cite{jackson2012social,banerjee2014gossip,microfinancedata} to examine the causal effect of belonging to an SHG on financial risk tolerance (measured as the presence of outstanding loans).
% , using 2010 survey data from 77 villages in Karnataka, India \cite{jackson2012social,banerjee2014gossip,microfinancedata}. 
The survey contains data about individuals in two forms: their social interactions with non-relatives (a toy example of the social network is shown Figure \ref{fig:socialnet}), along with information about each person (shown in Table \ref{tbl:covariates}). 
The information displayed in Table \ref{tbl:covariates} includes, for each person, the occupation of that person, whether they have an Election Card (an identity proof for Indian citizens), whether they have savings, whether they belong to an SHG, and whether they have outstanding loans. 
A causal inference algorithm can then estimate for each person, the effect of being in an SHG on having outstanding loans. This treatment effect is shown in the gray column in Table \ref{tbl:covariates}, where the units whose rows are colored blue have been positively affected by being in an SHG. 

Notice that there are three distinct values in the gray column, namely $0, 0.5$, and $1$, thus, there is heterogeneity in the treatment effect. 
% Consider persons $1$ and $4$. The treatment effect of person $1$ is $0$ while the treatment effect of person $4$ is $1$, thus, there is heterogeneity in the treatment effect. 
Furthermore, consider the Election Card column. All people with election cards have treatment effect $\leq 0.5$ (in particular, there are those with treatment effect $0$), while all people without them have treatment effect $\geq 0.5$  (in particular, there are those with treatment effect $1$). Thus, splitting the population into two groups: those with an election card and those without it will split the treatment effect as well. Thus, election card is an effect modifier. 

Suppose we are further interested in testing whether two other properties are effect modifiers: (1) interactions with people who work in Farm Labour and (2) being part of a triad (i.e., belong to a 3-clique). 
This requires analysis that goes beyond knowing the properties of each person, given in Table \ref{tbl:covariates}, 
% since we also have to know the information about their neighbors in the social network, the effect of the neighbors on each person, and the effect of the local network structure on each person. 
since we also have to consider the treatment effect of the neighbors of each person, and the effect of the local network structure on a person. 
\end{example}
% \begin{example}\label{ex:hyp_intro}
% Once the treatment effect has been estimated, 
% we are further interested in testing the following hypothesis about the data: are people who (1) have an election card, (2) who have interactions with people who work in Farm Labour and (3) are part of a triad (i.e., belong to a 3-clique), more likely to benefit from participating in an SHG?, i.e., are they more likely to not have an outstanding loan if they belongs to an SHG? 
% To test this hypothesis we need to consider three factors: the information of an individual, the information about their neighbors in the social network, and the network structure.
% \end{example}


% The researchers performing causal inference may further be interested in {\em understanding which covariates played a role in influencing the treatment effect}, or, formally, which covariates are effect modifiers \cite{hernan2010causal,vanderweele2007four}. 
% If the treatment effect changes across populations with different values of a covariate, this covariate is called an effect modifier. 
%The researchers performing causal inference may further be interested in understanding {\em how different groups in the population responded to the treatment}, or, formally, which covariates are effect modifiers \cite{hernan2010causal,vanderweele2007four}. Finding such effect modifiers can assist researchers to understand how to plan a policy (e.g., a vaccine rollout policy may change when knowing that children under $10$ are less affected by the vaccine), and, in general, identifying the factors that influence the outcome, which may become another form of treatment (e.g., in a vaccine efficacy trial, if people who do regular physical exercise are more benefited by the vaccine, researchers can then try to investigate the relation between the vaccine effect and physical exercise). 

In this paper we propose a novel framework for the estimation of treatment effect heterogeneity and detecting effect modifiers, tailored to causal inference in social networks. 
%  First, we formalize complex effect modifiers that may arise because of complex social interaction between the subjects, i.e., effect modifiers associated with the neighbors' covariates on the outcome and the network structure associated with each subject. 
First, we define a causal model for social networks that captures complex effect modifiers that may arise because of complex social interaction between the subjects, i.e., effect modifiers associated with the neighbors' covariates on the outcome and the network structure associated with each subject. 
% Second, we propose a novel hypothesis testing approach to  .... .   \babak{Flesh out the contributions here}
Second, we propose a novel hypothesis testing approach to based on the standard $I^2$ test \cite{higgins2003measuring} that accounts for neighbors' covariates and patterns in the social network. 
Third, we provide an algorithm for testing effect modifiers. The algorithm relies on ideas from graph theory to handle network patterns \cite{houbraken2014index} and ideas from relational causal inference to handle neighbors covariates \cite{DSalimiPKGRS20}. 
Finally, we perform experiments using both synthetic data (simulating a vaccine trial) and real data (the network demonstrated in our example), showing the our solution is able to detect the true effect modifiers and is relatively insensitive to high levels of noise. 
 
 \babak{Here brag about the importance of the analytics provided by your system} 
Using our framework researchers can create and test hypotheses about complex effect modifiers in terms of network features or network patterns. 
For example, whether agents might financially cooperate due to indirect reciprocity relying on social capital inherent \cite{righi2018social}. 
The analysis provided by our framework plays a critical role in (1) testing for the existence or lack of heterogeneous treatment effects, (2) identifying sub-populations
for which a treatment is effective or harmful, (3) Generalizing causal effect estimates obtained from an study sample to a target population. 
 
%Moreover, effect modifiers can assist researchers in learning about the transportability of the treatment across different population \cite{pearl2014external,hernan2010causal}, i.e., the ability to extrapolate causal effects computed in one population to another population.  Since the data collected comprises a social network, the effect modifiers can refer to the features of each unit, the features of its neighbors in the network, and the local structure of the network surrounding each unit. 


% \babak{Move the following to related work} A large body of work has been dedicated to devising ways to test statistical hypotheses (e.g., \cite{snyder1978hypothesis,xia2017hypothesis,LAROSA201581,shaffer1995multiple,list2019multiple,viechtbauer2007hypothesis}). In particular, previous work has proposed hypotheses tests for the heterogeneity of a population in a study \cite{viechtbauer2007hypothesis}. These include heterogeneity tests such as Cochran's Q \cite{cochran1954combination}, $H$ statistics, $R$ statistics, and $I^2$ \cite{higgins2002quantifying,higgins2003measuring}. 
% However, such tests are limited to discrete covariates and they do not take into account the context of the social network, i.e., the possible effect of the neighbors' covariates on the outcome and the network structure associated with each unit. In the context of our running example, existing tests cannot examine whether neighbors occupation and belonging to a 3-clique are effect modifiers. 

%{\em In this paper we propose a novel test for treatment effect modifiers tailored to causal inference in social networks}. 
\babak{I stopped here}
Next overview our contributions in more detail. 


\paratitle{Model and test:} Our criterion for testing possible effect modifiers is based on $I^2$ \cite{higgins2003measuring} but allows for (1) continuous covariates, (2) graph patterns and (3) summarized neighbors' covariates. 
For (1), we define our test using an integral over the covariate values. This models the test more accurately than the standard sum over the values. 
For (2), we define a desideratum for matching graph patterns to the subgraphs that include each unit in the social network. Intuitively, we define a graph pattern with a specific distinguished node and say that a graph pattern matches a subgraph of a unit if there is a subgraph isomorphism from the pattern to the subgraph where the distinguished node is mapped to the unit. 
For (3), since the number of neighbors of each unit in the network may be different, we build on the notions of covariate summary proposed in previous work \cite{DSalimiPKGRS20}. Given a covariate of a unit in the social network, we aggregate this covariate across all neighbors into a single summarized number (e.g., the percentage of neighbors who work as Farm Labour). 

\paratitle{Algorithms for testing:} We devise an algorithmic solution for testing hypothesized effect modifiers according to our criterion. The algorithms incorporate ideas from causal inference, hypothesis testing and graph theory. Namely, our solution uses causal inference to compute the treatment effect for each unit (conditional treatment effect) and subgraph isomorphism concepts (using the ISMAGS algorithm \cite{houbraken2014index}) to compute the value of the hypothesized effect modifier for each unit. 
Once these are computed, our solution estimates the influence of the covariate on the treatment effect using regression. 

\paratitle{Experimental study:} We provide an extensive experimental evaluation using a real social network based on a 2010 survey data from 77 villages in Karnataka, India \cite{jackson2012social,banerjee2014gossip,microfinancedata} (our running example) as well as synthetic data, simulating a vaccine efficacy trial. 
Through the synthetic data, we examine the effect of the number of units and the noise in the potential outcome on our test. 
Our results indicate that as the number of units increases (up to $4096$), the real effect modifiers
Through the real data, we demonstrate a use-case, showing our system's performance and its ability to find effect modifiers in a large scale network ($\sim$ 17K units). 

% In statistical studies, researchers often require tools for testing their hypotheses in an efficient and reliable manner.
% Hypothesis testing is therefore an important cornerstone in statistics and it has been studied in various settings and contexts (e.g., \cite{snyder1978hypothesis,xia2017hypothesis,LAROSA201581,shaffer1995multiple,list2019multiple}). There are multiple ways of testing hypotheses 
 

==> old/intro.tex <==
\section{Motivation}
Causal Inference has mostly been used to understand the effect of a previously made intervention or action on an outcome of interest. This line of causal inference is often termed as retrospective causal inference. However, often, the results of causal analysis has been used to make optimal choices that maximizes each individual's utility and minimizes the regret. The crucial part here will to be identify which individuals are benefited from a particular treatment choice and which individuals are not. In other words, the key along with causal inference is to understand heterogeneity of treatment effect in terms of covariates. If a decision maker were to use a system for high-stakes decision, it is very important for the system to be explanable/interpretable - so as to reason aobut why and which units are responding positively and negatively to a treatment of interest. 

In a classical setting, if we were to use linear modeling, matching or stratification based on observed covariates under SUTVA and strong ignorability, the treatment effect heterogeneity is trivially determined as a function of linear model or matched groups. Also, the explanation of effect heterogeneity in terms of effect modifiers is directly know from the method itself. However, if one had used a black-box method to estimate individualized treatment effects, then an interpretable prediction function such as linear model or decision trees can be fitted to to determine effect modifiers and their influence simultaneously and interpretably. 

% \babak{So, the target audience of our research could be both policy makers and system designers. We argue the causal mechanism learned for estimating individual treatment effect is a function of data and require explanation both for the purpose of debugging and policy management. We treat the covariate adjustment mechanism as a black-box and approximate aspects of it (say whether the effect is positive or negative for individuals) using a surrogate model which is both interpratable and facilitate generating local explanations (what I mean by this is an adjustment procedure could be interpratable but difficult to explain at the same time, say using the combination of matching for pre-processing and regression adjustment is interpratable but it is not easy to generate explanations without having a surrogate model that approximate the entire process). The surrogate model (say decision tree) shed light on the global properties of the learned function for estimating individual treatment, facilitates generating local explanations or can pinpoint to error in data (say outliers, selection bias, ...). Is that correct? In that case I think we need to study the fidelity of our surrogate model (which might be done only w.r.t particular adjustment procedures), e.g., to establish some approximation guarantee. This problem seems to be legit and interesting even in non-relational settings.}


% \amir{I think the above two para. are good for general background but aren't needed right now}

As a word of caution, it should be note that the association of effect modifying covariates and the treatment effect should not be misunderstood as causal relationship, i.e., change the effect modifying covariate for a unit in a certain direction might not change the true treatment effect of that unit in same direction as the sign of association. This approach primarily partitions the space and finds subspace where treatment effect is positive and/or negative. If the user is interested in understanding actionable recourse, then user must perform another causal study analyzing the effect of that particular intervention on the outcome of interest.

% \babak{ I want to push back on the above claim. See the followings:
% }

% Given a binary treatment variable $X \in \{x,x'\}$ the individual effect of $X$ on an outcome $Y$ for an individual with observed attributes $\bf{a}=\{a_1, \ldots, a_n\}$ reads as 
% $IE=E(y_{X \leftarrow x} \mid \bf{a})-E(y_{X \leftarrow x'} |\bf{a})$. Suppose IE is zero or negative for an individual $\bf{a}$. Let us define the problem of generating counterfactual explanation in terms of a unary covariate $A_i$ for the an individual $\bf{a}$ as the following optimisation problem: 

% {
% \begin{align} 
% \argmin_{\hat{a_i} \in Dom(A_i)} & cost(a_i,\hat{a_i}) \nonumber  \\
%  &  \hspace{-1cm } s.t. \ \    
% E(y_{X \leftarrow x } \mid {\bf a}_{A_i \leftarrow \hat{a_i}} )-E(y_{X \leftarrow x'} \mid  {\bf a}_{A_i\leftarrow \hat{a_i}})>0 
% \end{align}
% }
% Where, $\bf{a}_{A\leftarrow \hat{a_i}}$ denotes the profile of the user post intervention $A_i\leftarrow \hat{a_i}$. 

% \babak{The above optimisation problem prescribe a minimal intervention on a covariate (can be extended to a set of covariates) such that after the hypothetical intervention the individual get benefit from the policy $X \leftarrow x$. Notice that I formulated the problem in a way such that the same function used for estimating IE can be used for solving the above optimisation problem.  Using these counterfactual explanations, for example, for an author that receives no benefit from her prestige, we can generate explanations of the form "had the author were male and senior, her prestige would have been positively affected her paper acceptance rate, given that the author is a female and not senior. I think the problem makes sense but quite complicated in terms of estimation. However, I think it goes beyond the scope of this paper. }


Back to explaining heterogeneity - in relational setups, such as a social networks, firstly finding individualized treatment effect is very tricky due to contagion and interference, and secondly, {\em the explanation of treatment effect should not always be examined only in terms of the covariates on an edge or a node but also in terms of the relational structure in which the unit of interest exists}, e.g., effect of an individual's vaccination status on possibility of catching a disease is dependent on if their immediate social connection have been vaccinated or not along with the age and medical history of the individual. 
Such complex structures are usually not captured as covariartes by the unit table.
Thus, explaining heterogeneity in a relational setup is trickier than the classical setup. Summarizing and explaining relational structure interpretably might be even more challenging depending on the true nature of dependency e.g., explaining in terms of degree centrality of a node is relatively more interpretable compared to explaining in terms eigenvalue centrality of a node. 
% \babak{Our second contribution is to extend the analysis in the first phase to relational settings. By tracing back the explanations generated for the unit table (using the surrogate model) we would be able to related the learned causal mechanism to the base units and the underling relational structure.}

In this work, we intend to develop a framework which, given causal estimation methodology, generates rule-based explanation for heterogeneity in the treatment effect for different units of interest. These explanations aim to capture structural properties that are not present in the unit table. 
Our work aims to aid, for example, public health experiments on determining optimal vaccination strategy to minimize the spread of a disease such as covid-19. Another use case of our framework will be in an academic setting where the administration wants to find which students benefit from tutoring and which students don't.

\begin{example}
Consider a situation where the public health experts are interested in estimating the efficacy of a pharmaceutical intervention such as a drug. Due to the physiological differences across patients, each patient reacts to the drug differently. For instance, an older patient might react more to the drug than the younger counterpart. If the public health experts uses a highly flexible and black-box causal inference toolkit such as BART to estimate causal effects, then this heterogeneity across the population is captured while estimating conditional average treatment effects (CATE). However, due to the black-box nature of the toolkit, it is hard to infer the same from the results directly. For instance, if we were interested in explaining which units have positive treatment effect versus negative treatment effect, the we can learn a shallow decision tree to partition the space of estimated CATEs as a function of covariates (which are also effect modifiers). The shallow decision tree is a rule based system indicating the sign of treatment effect in each subspace partitioned by these rules. Now, consider the same for a situation where the units are in a social network and there is a possibility of contagion and interference. Again, a highly flexible toolkit as one described in \cite{ogburn, salimi, sherman} can be used to estimate CATE accurately. However, the experts intend also to learn the heterogeneity in an interpretable way in order to optimally assign treatment for maximal positive outcome. For instance, a simple case can that if a unit in a part of a triangle or a larger clique then it has higher probability of positive treatment effect. While the CATEs are accurately returned by causal inference toolkit, the heterogeneity might not be well explained as a function of egocentric simple network motifs and covariates. 
\end{example}

% \subsection{Example}
\begin{example}
Consider the social network depicted in Figure \ref{fig:socialnet}. The network simulates a vaccine trial on a group of subjects where the edges denote social contact. Additionally, each subject has covariates of $Age, Immunocompromised, BioSex$, shown in Table \ref{tbl:covariates}. The goal of the trial is to determine the efficacy of a vaccine. This network and the covariates of each subject, along with the query ``Does the new vaccine prevents infection?'' is inputted to a black-box causal model (e.g., BART \cite{...}). The output of the model is the treatment affect of the vaccine for each unit. In Figure \ref{fig:socialnet}, the green subjects are predicted to have high treatment affect. 
However, the experts intend also to learn {\em the reason for the heterogeneity in an interpretable way in order to optimally assign treatment for maximal positive outcome.}
Here, green units are part of triangle cliques, where the rest of the clique is composed of non-immunocompromised adults, implying that subjects who are part of adult social cliques may be more positively affected by the immunity provided by a vaccine. 
\end{example}


Consider a district of $n$ people, socially connected with each other. With the onset of an epidemic, the district officials want to design a strategy for the optimal vaccine allocation program to contain the spread. The public health officials uses the vaccination data from previous years' vaccine efficacy studies to understand which units have higher efficacy to vaccination and which units don't respond to vaccination. 

Figure~\ref{fig:socialnet} shows the example social network of district $\mathcal{G}$ with colors representing the intensity of treatment effect. The units colored in blue are one with low treatment effect and the one colored orange are the one with higher treatment effect. Public health officials, here, intend to find egocentric features of these orange nodes such as the network neighborhood features and features like age, gender and ethnicity. The idea is not only to mine these important features but public health experts also intend to develop optimal treatment policy using these results. 
% \begin{figure}
%     \centering
%     \includegraphics[width=0.48\textwidth]{figs/socialnet.png}
%     \caption{Social Network of the District, color-coded such that blue are one with low treatment effect and the one colored orange are the one with high treatment effect.}
%     \label{fig:socialnet}
% \end{figure}
\begin{figure}
    \centering
\begin{tikzpicture}
\begin{scope}[every node/.style={circle,thick,draw}]
    \node[fill=ForestGreen] (A) at (2,3) {A};
    \node[fill=ForestGreen] (B) at (0,3) {B};
    \node[fill=ForestGreen] (C) at (1,4) {C};
    
    \node[fill=ForestGreen] (D) at (6,3) {D};
    \node[fill=ForestGreen] (E) at (4,3) {E};
    \node[fill=ForestGreen] (F) at (5,4) {F};
    
    \node[fill=ForestGreen] (G) at (6,0) {G};
    \node[fill=ForestGreen] (H) at (4,0) {H};
    \node[fill=ForestGreen] (I) at (5,1) {I};
    
    \node (J) at (3,2.7) {J};
    \node (K) at (4,1.8) {K};
    \node (L) at (0,2) {L};
    \node (M) at (2,0.3) {M};
\end{scope}

\begin{scope}[>={Stealth[black]},
            %   every node/.style={fill=white,circle},
              every edge/.style={draw=red,very thick}]
    \path [-] (A) edge node {} (B);
    \path [-] (A) edge node {} (C);
    \path [-] (B) edge node {} (C);
    
    \path [-] (D) edge node {} (E);
    \path [-] (D) edge node {} (F);
    \path [-] (E) edge node {} (F);
    
    \path [-] (G) edge node {} (H);
    \path [-] (G) edge node {} (I);
    \path [-] (H) edge node {} (I);
    
    \path [-] (A) edge node {} (J);
    \path [-] (E) edge node {} (J);
    \path [-] (I) edge node {} (K);
    \path [-] (J) edge node {} (K);
    \path [-] (L) edge node {} (B);
    \path [-] (H) edge node {} (M);
    \path [-] (M) edge node {} (L);
    \path [-] (D) edge node {} (G);
    
\end{scope}
\end{tikzpicture}
    \caption{Network of social contacts. Green nodes have high treatment effect}\label{fig:socialnet}
\end{figure}

\begin{table}[h]
    \centering \footnotesize
    \caption{Covariates of the units in the social neetwork shown in Figure \ref{fig:socialnet}}\label{tbl:covariates}
    \begin{tabular}{| c | c | c | c |}
        \rowcolor[HTML]{C0C0C0} 
        \hline
        {\bf Subject} & 
        {\bf Age} &
        {\bf Immunocomp.} &
        {\bf BioSex}\\
        \hline
        \hline A & 45 & No & F \\
        \hline B & 35 & No & M \\
        \hline C & 38 & No & F \\
        \hline D & 20 & No & F \\
        \hline E & 22 & No & F \\
        \hline F & 25 & No & M \\
        \hline G & 26 & No & M \\
        \hline H & 28 & No & F \\
        \hline I & 30 & No & M \\
        \hline J & 10 & Yes & M \\
        \hline K & 11 & No & F \\
        \hline L & 8 & Yes & M \\
        \hline M & 8 & No & F \\
        \hline

    \end{tabular}
    \vspace{-3mm}
\end{table}

Consider a simpler case where each node has no covariates except the network ties. We want to find network feature(s) that discriminate between the blue and the orange nodes. In this case, for a network feature $\mathcal{F}$, we are interest in estimating the following quantities of interest, $\mathbf{E}\left[\tau_i ~|~ \mathcal{F} \in \mathcal{G}_i\right] $ or $P\left[\tau_i>\alpha ~|~ \mathcal{F} \in \mathcal{G}_i\right]$.

In this toy example, it is easy to notice from visual inspection that all the nodes which are part of a triangle are orange i.e. $\tau_i > \alpha$. This implies $P\left[ \tau_i > \alpha ~|~ \Delta \in \mathcal{G}_i\right] = P\left[ \text{color}_i = \text{orange} ~|~ \Delta \in \mathcal{G}_i\right] = 1$. As a public health official, in this case, providing.
\paragraph{Framework}

\begin{figure}
    \centering
    \includegraphics[width=\linewidth]{figs/framework2.png}
    \caption{Initial Framework}
    \label{fig:framework}
\end{figure}

Our framework is depicted in Figure \ref{fig:framework}. First, a social network graph (where the nodes are the units) and a causal query are inputted to a black-box causal model. The model outputs the treatment effect for each unit. Then, our solution automatically divides the space of units based on heterogeneity of treatment effect, according to covariates of the unit themselves, but also according to network features of these units (e.g., is the unit part of a clique) and the covariates of its neighbors (e.g., are all the neighbors of the unit adults). 

% Our framework is depicted in Figure \ref{fig:framework}. First, a social network graph (where the nodes are the units) and a causal query are inputted to a black-box causal model. The model outputs the treatment effect for each unit. Then, users may choose a subset of units with a common treatment affect (e.g., unit positively affected by the treatment) and ask the system to find their common properties based on their location in the network and their covariates (e.g., all units selected are the center nodes of a star graph and all of their neighbors in that graph have $age < 50$). 




==> old/intro_old.tex <==
\section{introduction}\label{sec:intro}
As Machine Learning and inference models progress in their complexity, there is a parallel line of work that aims to explain them and their properties \cite{...}. A notable such model is that of {\em causal inference} where the goal is to determine the cause and effect from the observed data. \amir{Continue}

Previous work \cite{DSalimiPKGRS20} has proposed a model for relational causal learning, where the data used for the inference is stored in a relational database, possibly containing multiple tables and a complex schema. This model ties together the standard manner in which data is stored and the process of causal inference. 
The framework is based on a relational database and a set of rules specifying background knowledge. Applying these, users can formulate causal queries and get their results. 
However, users who get such result may further be interested in the reason for such results, particularly, if the result is unexpected. 


\begin{figure}[!htb]
    \centering \footnotesize
    \begin{minipage}{.5\linewidth}
        \centering
        \caption*{Authors}\label{tbl:authors}
        \begin{tabular}{ c | c | c | c | c | c |}
           \cline{2-4} & {\bf person} & {\bf prestige} & {\bf qualification} \\
            \hline $a_1$ & Bob & 1 & 50 \\
            \hline $a_2$ & Carlos & 0 & 20 \\
            \hline $a_3$ & Eva & 1 & 2 \\
            \hline
        \end{tabular}
    \end{minipage}%
    \begin{minipage}{.5\linewidth}
        \centering
        \caption*{Submissions}\label{tbl:submissions}
        \begin{tabular}{ c | c | c | c | c | c |}
            \cline{2-3} & {\bf sub} & {\bf score} \\
            \hline $s_1$ & $s1$ & 0.75 \\
            \hline $s_2$ & $s2$ & 0.4 \\
            \hline $s_3$ & $s3$ & 0.1 \\
            \hline
        \end{tabular}
    \end{minipage}
    \begin{minipage}{.33\linewidth}
        \centering
        \caption*{Authorship}\label{tbl:authorship}
        \begin{tabular}{c | c | c | c | c | c |}
            \cline{2-3} &  {\bf person} & {\bf sub} \\
            \hline $as_1$ & Bob & s1 \\
            \hline $as_2$ & Eva & s1 \\
            \hline $as_3$ & Eva & s2 \\
            \hline $as_4$ & Eva & s3 \\
            \hline $as_5$ & Carlos & s3 \\
            \hline
        \end{tabular}
    \end{minipage}%
    \begin{minipage}{.33\linewidth}
        \centering
        \caption*{Submitted}\label{tbl:submitted}
        \begin{tabular}{c | c | c | c | c | c |}
            \cline{2-3} & {\bf sub} & {\bf conf}\\
            \hline $sc_1$ & s1 & confDB \\
            \hline $sc_2$ & s2 & confAI \\
            \hline $sc_3$ & s3 & confAI \\
            \hline
        \end{tabular}
    \end{minipage}%
    \begin{minipage}{.33\linewidth}
        \centering
        \caption*{Conferences}\label{tbl:conferences}
        \begin{tabular}{c | c | c | c | c | c |}
            \cline{2-3} & {\bf conf} & {\bf blind}\\
            \hline $c_1$ & confDB & single \\
            \hline $c_2$ & confAI & double \\
            \hline
        \end{tabular}
    \end{minipage}
    \caption{Review database instance $\mathcal{D}$}\label{fig:db}
    % \vspace{-6mm}
\end{figure}

\begin{table}[]
    \centering \footnotesize
    \caption{The unit table for $T[X] = Prestige[A]$ and $Y[X'] = AVG\_Score[A]$ based on Figure \ref{fig:db}}\label{tbl:unit_tbl}
        \begin{tabular}{|c | c | c | c | c | c |}
           \hline {\bf Unit} & {\bf Outcome} & \begin{tabular}{@{}c@{}}{\bf Embedded coauthors'}\\ {\bf treatment}\end{tabular} & \multicolumn{2}{c|}{\begin{tabular}{@{}c@{}}{\bf Embedded collaborators’}\\ {\bf covariates}\end{tabular}}\\
           \hline Author ID & AVG\_score & \begin{tabular}{@{}c@{}}Prestige\\ (AVG)\end{tabular} & \begin{tabular}{@{}c@{}}Centrality\\ (COUNT)\end{tabular} & \begin{tabular}{@{}c@{}}H-index\\ (AVG)\end{tabular} \\
            \hline Bob & 0.75 & 1 & 1 & 2 \\
            \hline Carlos & 0.1 & 1 & 1 & 2 \\
            \hline Eva & 0.41 & 0.5 & 2 & 35 \\
            \hline
        \end{tabular}
\end{table}


\begin{table}[]
    \centering \footnotesize
    \caption{The unit table for $T[X] = Prestige[A]$ and $Y[X'] = AVG\_Score[A]$ based on Figure \ref{fig:db} without the tuple $a_2$. Cahnges from the Table \ref{tbl:unit_tbl} are marked in blue \amir{Not sure what centrality is}}\label{tbl:unit_tbl_deleted}
        \begin{tabular}{|c | c | c | c | c | c |}
           \hline {\bf Unit} & {\bf Outcome} & \begin{tabular}{@{}c@{}}{\bf Embedded coauthors'}\\ {\bf treatment}\end{tabular} & \multicolumn{2}{c|}{\begin{tabular}{@{}c@{}}{\bf Embedded collaborators’}\\ {\bf covariates}\end{tabular}}\\
           \hline Author ID & AVG\_score & \begin{tabular}{@{}c@{}}Prestige\\ (AVG)\end{tabular} & \begin{tabular}{@{}c@{}}Centrality\\ (COUNT)\end{tabular} & \begin{tabular}{@{}c@{}}H-index\\ (AVG)\end{tabular} \\
            \hline Bob & 0.75 & \cellcolor{blue!25}0 & 1 & \cellcolor{blue!25}0 \\
            \hline Carlos & 0.1 & \cellcolor{blue!25}0 & 1 & \cellcolor{blue!25}0 \\
            \hline
        \end{tabular}
\end{table}


\begin{example}\label{ex:motivation}
Consider the review database in Figure \ref{fig:db} (the annotation on each tuple appears on its righthand side) and the following causal rules, stating background knowledge: 
\begin{small}
\begin{enumerate}
    \item Prestige[A] $\Leftarrow$ Qualification[A] WHERE Person(A)
    \item Quality[S] $\Leftarrow$ Qualification[A], Prestige[A] WHERE Author(A, S)
    \item Score[S] $\Leftarrow$ Prestige[A] WHERE Author(A, S)
    \item Score[S] $\Leftarrow$ Quality[S] WHERE Submission(S)
\end{enumerate}
\end{small}
When inputted to the CaRL system \cite{DSalimiPKGRS20}, along with the causal query ``Score[S] $\Leftarrow$ Prestige[A]?'', the result is the ATE of author prestige on the submission score, which is $1.1$. However, a user who gets this result may wonder why is this ATE so high or low? (i.e., why is there a high/low bias?) or what are the most influential authors and submission? 
\end{example}

Explaining the results of complex systems using source tuples has been studied in multiple different settings, such as database queries \cite{...} and ML models \cite{...}. 
However, in the relational causal inference framework, the combination of the complex structure of the relational databases and the various transformations the data undergoes to compute the result of the causal query often leads to scenarios where different tuples may have different effects over the result. 
For example, the absence of a tuple from the database may be negligible when it comes to the result of the query, while the absence of a different tuple may dramatically change it. Moreover, a removal of some tuples may both remove rows from the unit table and change the cells of others. 


\begin{example}
Consider the effect of the tuple $a_2$ (the Author tuple of Eva). To measure its effect, suppose it is absent from the database. 
This would change various cells in the unit table in Table \ref{tbl:unit_tbl}. The updated cells are shown in blue in Table \ref{tbl:unit_tbl_deleted}. Beyond removing a row of the table, the absence of $a_1$ has also changed cells related to other author authors. The effect of other tuples, such as $s_1$, will not cause the removal of rows from the table, but will cause changes in more cells (such as Bob's AVG\_Score). 
\end{example}

% \amir{Join paths of deletion can also be of interest here, i.e., removing $a_1$ necessarily removes $as_3$ and $s_2$ which can cause more changes}

This poses a challenge of evaluating the influence of source tuples on the result of a causal query. 
% \amir{what about removing control tuples? add a constraint forbidding it?}
% \amir{Another challenge of course: efficiently compute the influence without retraining}

==> old/matching.tex <==
\section{Finding Explanations for Matching}
Our first proposed solution is for the case where matching methods are used to compute the result from the unit table. These can be modeled, in the relational database setting, as aggregate queries. Therefore, our algorithm will rely on these to compute the most influential set of tuples. 



==> old/model.tex <==
\section{model and Assumptions}\label{sec:model}

\subsection{Notations and Assumptions}

\begin{table}[!htb]
% \vspace{-3mm}
\centering
\caption{Notations \amir{add more if needed}}\label{notations}
\begin{tabular}{| c | l | c |}
\hline $G$ & Social Network with \\
\hline $E_{i,j}$ & Random indicator variable of a tie between $i$ and $j$ \\
\hline $X_i$ & Vector of random variables of the covariates for unit $i$ \\
\hline $T_i$ & Treatment/intervention choice for unit $i$ \\
\hline $Y_i$ & Observed outcome for unit $i$ \\
\hline $Y(t,t_{n,i})$ & Potential outcome unit under the treatment choice $t$ and the neighbors’ treatment choice $t_{n,i})$ \\
\hline
\end{tabular}
%\vspace{-2mm}
\end{table}

\amir{This should be written more formally.}
In this section, we discuss the notations that we use in the paper to discuss the problem of interest and its solution. Next we also discuss the assumption under which we study the research question. We consider a setup with a network of nodes and ties, where each node corresponds to a unit of interest in our dataset. For instance, these nodes can correspond to patients or civilians in a social network, or cities connected via a transportation network. The network $R$ is represented as the union of set of nodes $V$ and ties $E$. Thus $E_{i,j}$ represents the random variable for tie between units $i$ and $j$ in $V$. Each of these nodes have their own properties denoted by a vector covariates that includes age of patient or population of a city. The vector of random variables corresponding to the covariates for unit $i$ is denoted as $X_i$. Further, $T_i$ is the treatment/intervention choice for node $i$, and $Y_i$ is the observed outcome for node $i$. In this study, we consider that researchers use a black-box causal effect estimation approach to estimate the effect of intervention $T$ on outcome $Y$. However, causal inference in a network scenario is need additional considerations because of the following three reasons:
\begin{enumerate}
    \item The ego-centric network structure can be a confounder/effect modifier. In this case, one needs to control for network structures to estimate the effects.
    \item The treatment effects can spillover from neighboring units to the unit of interest which can contaminate the estimated effects, if the information of neighbors treatment choices are not taken into account.
    \item Contagious effect can further introduce complication where the outcome of one unit is determine by/correlated with the outcome of the neighboring unit such as in the case of Covid-19 infections.
\end{enumerate}
Methodologists have come up with sophisticated tools to estimate individualized treatment effects in each of these cases \amir{cite?}. However, using these tools might be perceived as black-box by the applied scientists. In this work we aim at explaining the heterogeneity in these estimates of treatment effects. This aims to aid optimal treatment policy for the decision makers using the explanations.We divide our analysis for each of these cases and lastly, also provide a unified approach for all. 

\amir{Every assumption here needs justification/citation from previous work:}We assume that only the immediate neighbors and network connections affect the random variables of an unit. The second or higher order connections and network ties can thus be ignored while analyzing and explaining the effects. $E_{i,\cdot}$ represents the ties incident on unit $i$ and $V_{i}$ represents the neighbors of unit $i$ i.e. if $E_{i,j} = 1$ then $j \in V_i$. The analysis also hinges on the assumption that $X_i$ is identically drawn from distribution $\mu(X)$ for all $i \in V$. If $E_{i,j}=0$ then $X_i \perp X_j$. However, if $E_{i,j}=1$ then $X_i$ might not be independent of $X_j$. We make the unit homogeneity assumption such that unit $i$ and unit $j$ for all $i$ and $j$ have identical interpretation. Further, we also make edge/tie homogeneity assumption stating $E_{i,j}$ has same interpretation for all $i$ and $j$ in $V$. 

Our notation follows Rubin's potential outcome framework \amir{cite?} where $Y_i(t;\overline{t_{V_i}})$ is the potential outcome for unit $i$ under treatment choice $t$ such that the treatment assignment vector for the neighbors of $i$ is equal to $\overline{t_{V_i}}$. 
We assume strong ignorability to enable estimation: $Y_i(t;\overline{t_{V_i}}) \perp T_i | X_i, E_{i,\cdot}, \overline{T_{V_i}}=\overline{t_{V_i}}$

\subsection{Explanation Patterns}
We define the concepts of a relational database, relational causal DAG, and a causal query. We then turn to defining explanations for such queries.

% \begin{definition}[Covariate-base decision tree]
% \amir{formalize the definition}
% \end{definition}

\begin{definition}[Distinguishing Explanation Pattern]\label{def:distinguishing_explanation}
Given a social network graph $G = (V,E)$ and a set of units $S \subseteq V$, an explanation pattern $P$ is a graph such that $\forall v_i \in S~ \exists f_i: G_i \to P$, where $G_i$ includes $v_i$ such that $f_i$ is an isomorphism and there is a node $u \in P$ such that $f_i(v_i) = u$. 
Each such $f_i$ is called {\em pattern-preserving isomorphism of $S$}. 
Given a social network graph $G = (V,E)$ and a set of units $S \subseteq V$, a {\em distinguishing explanation pattern} $P$ is a pattern-preserving isomorphism of $S$ such that $\forall v_i \in V\setminus S~ \not\exists f_i: G_i \to P$.  
% Given a social network graph $G = (V,E)$ and a set of units $S \subseteq V$, an explanation pattern $P$ is a graph such that (1) $\forall v_i \in S~ \exists f_i: G_i \to P$, where $G_i$ includes $v_i$ such that $f_i$ is an isomorphism and there is a node $u \in P$ such that $f_i(v_i) = u$. 
% Each such $f_i$ is called {\em pattern-preserving isomorphism}
% and (2) $\forall v_i \in V\setminus S~ \not\exists f_i: G_i \to P$.  
\end{definition}

This definition subsumes and generalizes the notion of structural equivalence \cite{wasserman1994social}, previously devised in the context of causal inference on social networks.

% \amir{I think for start we can just consider the maximum distinguishing subgraph and then expand to weighted graphs with weights on the edges representing the strength of the connection, like in the influence maximization literature. Also incorporate the neighbor covariates in the second step}



% \begin{definition}[Causal rules, from \cite{RoyS14}]
% \amir{take the definition from \cite{RoyS14}, basic $\Delta$ rules, e.g. $\Delta(pid, title, aid) \gets \Delta(aid, name, oid), WrittenBy(aid,pid)$ (if an author is deleted, delete the papers written by this author)}
% \end{definition}

% \begin{definition}[Influencing set]
% Given a database $D$, a unit table $T_U$, a set of causal rules $\mathcal{P}$, and a covariate-based decision tree $T = (V,E)$ over $T_U$, denote by $v\in V$ the node representing the most influenced units by the treatment, i.e., the node with the highest value, an influencing set is a set $S\subseteq D$ such that $\mathcal{P}(D \setminus S)$ causes the removal of all units represented in $v$. 
% \end{definition}

% \begin{definition}[Side-effect of an influencing set]
% Given a database $D$, a unit table $T_U$, a set of causal rules $\mathcal{P}$, a covariate-based decision tree $T = (V,E)$ over $T_U$, denote by $v\in V$ the node representing the most influenced units by the treatment, i.e., the node with the highest value, and an influencing set $S$, the side-effect of $S$ is defined as:
% $$ se(S) = \sum_{u\neq v, u \in V} Removed(u, D, S, \mathcal{P}) $$
% where $Removed(u, D, S, \mathcal{P})$ is the number of units removed from $u$ by removing $\mathcal{P}(D \setminus S)$ from $D$. 
% \end{definition}

% \begin{definition}[Minimum side-effect influencing set]
% Given a database $D$, a unit table $T_U$, a set of causal rules $\mathcal{P}$, and a covariate-based decision tree $T = (V,E)$ over $T_U$, denote by $v\in V$ the node representing the most influenced units by the treatment, the minimum side-effect influencing set is an influencing set $S\subseteq D$ with the minimum side-effect.
% \end{definition}

% \amir{Finding the minimum side-effect influencing set is NP-hard by reduction from \cite{BunemanKT02} since the decision tree can be thought of as a complicated view that was generated using projections, joins, and aggregates}

% \amir{All previous work on deletion propagation has focused on CQs and versions thereof, so no immediate solution to our problem}

% \amir{Possible heuristic algorithm for finding the minimum side-effect influencing set: start from the base table of the units that we wish to remove and backtrack using the causal rules to find the minimum entities to remove so that the units are removed. Use a balance function between the number of units removed from the interesting node (which we want to maximize) and the number of units removed from other nodes (which we want to minimize).}

% \amir{Another approach for finding the minimum side-effect influencing set: consider the aggregate provenance and find the subset of entities in the prov. of the relevant vertex that has the minimum side-effect using a SAT solver.}

% \begin{definition}[Predicate explanation]
% Given a database $D$, a unit table $T_U$, a set of causal rules $\mathcal{P}$, a covariate-based decision tree $T = (V,E)$ over $T_U$, and a minimum size influencing set $S$, a predicate explanation $\Phi$ is a conjunction of predicates of the form $A \circ c$ where $\circ \in \{<, >, =, \neq, \leq, \geq\}$ such that $t\in S$ iff $\Phi(t) = true$. 
% \end{definition}

\subsection{Problem Statement}
Causal inference methods are used to estimate average (ATE) and conditional average treatment effects (CATE) for understanding the effect of an intervention of interest on a specific outcome for e.g. effect of vaccination on propensity of catching a disease. In potential outcome framework, the treatment effects are defined as the contrast of potential outcomes under different treatment choices given everything else is as it is (ceteris paribus). In a classical setting where the outcome and the treatment are only affected by the covariates of a unit i

If the conditional average treatment effects for any two different levels of covariates \amir{levels of covariates?} is not identical then the treatment effects are heterogeneous. 
$$\text{CATE:}\ \ \ \tau(x) = \mathbf{E}[y(1) - y(0) | X=x]$$
If there exist $x_1 \neq x_2$ such that $\tau(x_1)\neq\tau(x_2)$ then the treatment effects are heterogeneous.
If the research believes that the causal effects might be different across each individual, then they choose to use more flexible methods that allow estimating causal effects for each level of covariates. These estimated CATEs are typically real-valued numbers corresponding to what is the effect of intervention on the outcome for a given covariate level. However, in a lot of case, the researchers are interested in more coarser levels of heterogeneity i.e. the treatment effect for certain group is positive or negative (or null). 
In this study, we consider discretized treatment effect estimates such as positive vs negative, high vs low or multiple levels from 1 to k of treatment effects for each unit. 

\begin{definition}[Conditional Direct Effect]
Let $Y(t,t_n)$ be the potential outcome unit under the treatment choice $t$ and the neighbors' treatment choice $t_n$. Then, the conditional direct effect (CDE) is
 $\tau_i = \mathbf{E}\left[ Y(1,t_{n,i}) - Y(0,t_{n,i}) | W = w_i \right]$ where $w_i = \phi(x_i, n_{i}, g_i)$ stands for a non-parametric embedding $\phi$ \amir{explain ``non-parametric''}.
\end{definition}

\begin{example}
\amir{add the vaccine example}
\end{example}

\begin{definition}[Social network heterogeneity partition]
Given the conditional direct effect $\tau_i$ for each unit (node) $i$ in a social network $G$ using a black-box causal inference method, and a threshold $\tau_0$, 
% \amir{can also be expectation without a threshold}, 
the {\em \prob} problem is to find $x, n, g$ for all units $i\in G$ such that $\prod_i Pr(\tau_i > \tau_0~|~ x, n, g)$ is maximized, where $x$ is a covariate vector of a unit $i$, $n$ is a covariate vector of the neighbors of unit $i$, and $g$ is an explanation pattern.
\end{definition}

Intuitively, we are interested in the set of unit covariates, neighbor covariates and graph pattern that contributes to heterogeneity. 

\begin{example}\label{ex:prob}
Reconsider our running example with the network in Figure \ref{fig:socialnet} and the covarites in Table \ref{tbl:covariates}. If we set $\tau_0 = 0.5$ \amir{calculate the actual $\tau_0$}, $x = (Immunocomp. = No)$, $n = (Immunocomp. = No)$, and $g = \Delta$ (a triangle pattern), we maximize $\prod_i Pr(\tau_i > 0.5~|~ x, n, g)$ since for every unit $i$, we have $Pr(\tau_i > 0.5~|~ x, n, g) = 1$ \amir{verify}. Thus, setting $x,n,g$ as above is the solution to \prob\ in this case. 
\end{example}

The decision problem version of \prob\ is that given $x, n, g$, verify whether it maximizes $\prod_i Pr(\tau_i > \tau_0~|~ x, n, g)$. 

\begin{proposition}
The decision problem version of \prob\ is NP-hard. 
\end{proposition}

\begin{proof}[Proof Sketch]
By reduction from subgraph isomorphism. Given a graph $G = (V,E)$ and a pattern $p$ we define the social network $G$ with empty covariates for every unit $v\in V$. Using a black-box causal inference method, and a threshold $\tau_0$, we need to check whether $p$ maximizes $\prod_i Pr(\tau_i > \tau_0~|~ p)$, i.e., we need to find whether $p$ is a distinguishing explanation pattern (Definition \ref{def:distinguishing_explanation}). \amir{continue}
\end{proof}
% \textbf{Problem Statement.} Given the treatment effects for each unit (node) in the social network using a highly flexible and powerful black-box causal inference method, we are interested in finding which features of the node, the neighbors of the node and their ties contribute towards the heterogeneity in treatment effects. 


==> old/model_old.tex <==
\section{model}\label{sec:model}
We define the concepts of a relational database, relational causal DAG, and a causal query. We then turn to defining explanations for such queries.


\amir{Just the needed defs for now}


\begin{figure}[h]
    \centering
    \includegraphics[width=\linewidth]{figs/carl_framwork.png}
    \caption{CaRL framework}
    \label{fig:carl}
\end{figure}

% We start by defining 

\begin{definition}[Explanation Query, from \cite{RoyS14}]
Given a database $\mathcal{D}$, a causal query $Q$ and a set of causal rules $\mathcal{C}$, an explanation query is a direction $dir \in \{low, high\}$. 
\end{definition}

Intuitively, an explanation query $low$ means that `the outputted value is unexpectedly low', so our goal is to explain why this is the case. The case for $dir = high$ is symmetric. 

\begin{example}\label{ex:explanation_query}
Reconsider the Database in Figure \ref{fig:db} and the causal rules and query presented in Example \ref{ex:motivation}. As explanation query is ``why is the ATE of prestige on score is so high?''. Formally, this query is modeled simply as $high$. 
\end{example}

The next definition relates to the degree that a specific version of the unit table helps in explaining the unexpected result.  

\begin{definition}[Table Degree]
Given a unit table $T$, an ATE value $v$, and an explanation query $dir$, the function $TD: 2^T \to \mathbb{R}$ is defined as follows:
% $$
% TD_{v,dir}(T) =
% \left\{
% 	\begin{array}{ll}
% 		1  & \mbox{if } dir \equiv `high' ~and~ ATE(T) < v \\
% 		1  & \mbox{if } dir \equiv `low' ~and~ ATE(T) > v \\
% 		0 & \mbox{else }
% 	\end{array}
% \right.
% $$
$$
TD_{v,dir}(T) =
\left\{
	\begin{array}{ll}
		v - ATE(T) & \mbox{if } dir \equiv `high' \\
		ATE(T) - v  & \mbox{if } dir \equiv `low'
	\end{array}
\right.
$$
\end{definition}

$TD$ defines the contribution of a unit table version to the explanation by giving a positive score to versions that change the ATE value to a more expected one. We are now ready to define the Shapley value of a unit cell. 

\begin{definition}[Shapley value of a unit cell]
Given a unit table $T$, and a cell from $T$, $c$, the Shapley value $c$ is defined as:
\begin{equation*}\label{eq:cellsEq}
\begin{split}
\varphi(c) = \mathlarger{\sum}_{S\subseteq T\setminus \{c\}}
\frac{|S|!(|T|-|S|-1)!}{|T|!}\cdot (TD_{v,dir}(S\cup \{c\}) - TD_{v,dir}(S))
\end{split}
\end{equation*}
where $S\subseteq T$ means that any cell of $T$ not in $S$ is given a `null' value \amir{makes sense in terms of causality?}.
\end{definition}



% \begin{definition}[Explanation Candidate, from \cite{RoyS14}]
% A candidate explanation $\phi$ is a conjunction of predicates on attributes: $\phi = \land_j \phi_j$ , where each $\phi_j$ is
% an atomic predicate of the form $\phi_j = [R_i.A~op~c]$, where $A$
% is an attribute of $R_i$, $c$ is a constant, and $op \in \{=, <, \leq, >, \geq\}$.
% \end{definition}

% In the next definition we use the concept of aggregate provenance \cite{AmsterdamerDT11} for the unit table cells. 


\begin{definition}[Unit Cell Provenance]
Given a database $\mathcal{D}$, a causal query $Q$ and a set of causal rules $\mathcal{C}$, Denote by $\mathcal{T}_U$ the unit table w.r.t. $\mathcal{D}$, $Q$, and $\mathcal{C}$. Let $c \in \mathcal{T}_U$ be a cell in $\mathcal{T}_U$. Then, the provenance of $c$, denoted by $prov(c)$, is the aggregate provenance of $c$. \amir{Is aggregate provenance enough or should we add references to the causal graph if it is changed?}
\end{definition}

\begin{example}\label{ex:provenance}
Consider the cell AVG\_Score in the third line of table \ref{tbl:unit_tbl}. Its unit cell provenance is composed of the tuples $s_1, s_2$ and $s_3$, where the formal expression, based on \cite{AmsterdamerDT11}, is $(s_1 \tens{} 0.75 + s_2 \tens{} 0.4 + s_3 \tens{} 0.1) / (s_1 \tens{} 1 + s_2 \tens{} 1 + s_3 \tens{} 1)$, where $\tens{}$ stands for the tensor product of annotations with values \amir{verify}. Assigning $s_i = 0$ represents the absence of $s_i$ and assigning $s_i = 1$ represents its presence. 
\end{example}

\paragraph*{Basic Algorithm:}
Given a database $D$, a unit table $T$, an ATE value $v$, and an explanation query $dir$:
\begin{itemize}
    \item Find the top-$k$ cells in $T$ with the highest Shapley values w.r.t. $v$ and $dir$
    \item Find the set of provenance tuples of these cells, $\mathcal{P} \in D$
    \item Check if deleting $\mathcal{P}$ induces more changes in $T$
    \item If no, return $\mathcal{P}$ as a set of predicates
    \item If yes, \amir{?}
\end{itemize}

{\bf Advantage:} No need to re-train.

{\bf Disadvantage:} Since this is backtracking, no guarantee that the set of source tuples does not change the unit table in other ways.

Alternatively, we can define the Shapley value on the source tuples themselves. 

\begin{definition}[Database Degree]
Given a database $D$, an ATE value $v$, and an explanation query $dir$, the function $DD: 2^D \to \mathbb{R}$ is defined as follows:
% $$
% DD_{v,dir}(D) =
% \left\{
% 	\begin{array}{ll}
% 		1  & \mbox{if } dir \equiv `high' ~and~ ATE(D) < v \\
% 		1  & \mbox{if } dir \equiv `low' ~and~ ATE(D) > v \\
% 		0 & \mbox{else } 
% 	\end{array}
% \right.
% $$
$$
DD_{v,dir}(D) =
\left\{
	\begin{array}{ll}
		v-ATE(D)  & \mbox{if } dir \equiv `high' \\
		ATE(D)-v  & \mbox{if } dir \equiv `low' 
	\end{array}
\right.
$$
\end{definition}

\begin{definition}[Shapley value of a database tuple]
Given a database $D$, and a tuple from $D$, $t$, the Shapley value $t$ is defined as:
\begin{equation*}\label{eq:cellsEq}
\begin{split}
\varphi(t) = \mathlarger{\sum}_{S\subseteq D\setminus \{t\}}
\frac{|S|!(|D|-|S|-1)!}{|D|!}\cdot (DD_{v,dir}(S\cup \{t\}) - DD_{v,dir}(S))
\end{split}
\end{equation*}
\end{definition}

% \paragraph*{Influence Function over the Unit Table}
% We introduce the concept of influence functions \cite{KohL17,WuF0W20}. Given an ML model, the idea is to measure the effect of changing a data point in the training set on the result of the model. 
% Let $\mathcal{T}_U$ be a unit table and let $M$ be an ML model parameterized by $V_M$ and with a loss function $L(V_M) = \frac{1}{n}\sum_{i=1}^n \ell(z_i, V_M)$. A change in a tuple of $\mathcal{T}_U$, $u \mapsto u'$, can be modeled as $arg\_min_{V_M}\{L(V_M) - L(u, V_M) + L(u', V_M)\}$. 
% Previous works \cite{cook1980characterizations,KohL17} have showed that the change is given by \amir{write expression}, denoted by $\mathcal{I}_{up,loss}(u, u')$.

% \begin{example}
% \amir{Continue Example \ref{ex:provenance} and measure the effect of the absence of $s_1$ with an influence function}
% \end{example}

% Abusing notation, we denote by $t\in prov(c)$ that a tuple $t \in \mathcal{D}$ (a tuple from the database) is in the provenance expression of a cell $c$ in the unit table $\mathcal{T}_U$ (e.g., in Example \ref{ex:provenance}, the tuple $s_1 \in prov(t_1[AVG\_Score])$ where $t_1$ is the first tuple in Table \ref{tbl:unit_tbl}). We draw on \cite{RoyS14} for the next definition, quantifying the effectiveness of a candidate explanation. 

% \begin{definition}[Degree of Explanation]
% Let $\mathcal{D}$ be a database, let $Q$ a causal query, let $\mathcal{C}$ be a set of causal rules, let $dir$ be an explanation query, and let $\mathcal{T}_U$ be a unit table. The degree of a candidate explanation $\phi$ is defined as 
% $$\sum_{\substack{u \in \mathcal{T}_U \\ c\in u}}\sum_{\substack{\phi(t) = True,\\t \in prov(c)}}\mathcal{I}_{up,loss}(u, u')$$
% i.e., the approximation of the change in ATE if $u$ is changed to $u'$ due to the removal of a tuple in the provenance of its cell $c$. \amir{not sure whether it should be sum of something else. Is there a paper on influence functions of sets of points?}
% \end{definition}


% \begin{example}
% Reconsider the explanation query in example \ref{ex:explanation_query}. The degree of an explanation $[Authors.person=Eva]$ is the approximated change in ATE when the tuple $a_3$ is deleted from the database, causing the unit table to change from the original (Table \ref{tbl:unit_tbl}) to Table \ref{tbl:unit_tbl_deleted}. \amir{Formalize. what is the corrected ATE?}
% \end{example}

% \amir{Other versions: (1) changing assumptions, (2) changing the query}



==> old/old_running_example.tex <==
\begin{figure}
    \centering
\begin{tikzpicture}
\begin{scope}[every node/.style={circle,thick,draw}]
    \node[fill=ForestGreen] (A) at (2,3) {A};
    \node[fill=ForestGreen] (B) at (0,3) {B};
    \node[fill=ForestGreen] (C) at (1,4) {C};
    
    \node[fill=ForestGreen] (D) at (6,3) {D};
    \node[fill=ForestGreen] (E) at (4,3) {E};
    \node[fill=ForestGreen] (F) at (5,4) {F};
    
    \node[fill=ForestGreen] (G) at (6,0) {G};
    \node[fill=ForestGreen] (H) at (4,0) {H};
    \node[fill=ForestGreen] (I) at (5,1) {I};
    
    \node (J) at (3,2.7) {J};
    \node (K) at (4,1.8) {K};
    \node (L) at (0,2) {L};
    \node (M) at (2,0.3) {M};
\end{scope}

\begin{scope}[>={Stealth[black]},
            %   every node/.style={fill=white,circle},
              every edge/.style={draw=red,very thick}]
    \path [-] (A) edge node {} (B);
    \path [-] (A) edge node {} (C);
    \path [-] (B) edge node {} (C);
    
    \path [-] (D) edge node {} (E);
    \path [-] (D) edge node {} (F);
    \path [-] (E) edge node {} (F);
    
    \path [-] (G) edge node {} (H);
    \path [-] (G) edge node {} (I);
    \path [-] (H) edge node {} (I);
    
    \path [-] (A) edge node {} (J);
    \path [-] (E) edge node {} (J);
    \path [-] (I) edge node {} (K);
    \path [-] (J) edge node {} (K);
    \path [-] (L) edge node {} (B);
    \path [-] (H) edge node {} (M);
    \path [-] (M) edge node {} (L);
    \path [-] (D) edge node {} (G);
    
\end{scope}
\end{tikzpicture}
    \caption{Network of social contacts. Green nodes have high treatment effect}\label{fig:socialnet}
\end{figure}

\begin{table}[h]
    \centering \footnotesize
    \caption{Unit table of the social network shown in Figure \ref{fig:socialnet}}\label{tbl:covariates}
    \begin{tabular}{| c | c | c | c | c | c |}
        \rowcolor[HTML]{C0C0C0} 
        \hline
        {\bf Subject} & 
        {\bf Age} &
        {\bf Immunocomp.} &
        {\bf BioSex} &
        {\bf Vaccinated} & 
        {\bf Infected} \\
        \hline
        \hline A & 45 & No & F & Yes & No \\
        \hline B & 35 & No & M & Yes & No \\
        \hline C & 38 & No & F & No & No \\
        \hline D & 20 & No & F & Yes & No \\
        \hline E & 22 & No & F & No & No \\
        \hline F & 25 & No & M & Yes & No\\
        \hline G & 26 & No & M & Yes & No \\
        \hline H & 28 & No & F & Yes & No \\
        \hline I & 30 & No & M & Yes & No \\
        \hline J & 10 & Yes & M & No & Yes \\
        \hline K & 11 & No & F & Yes & No \\
        \hline L & 8 & Yes & M & No & Yes \\
        \hline M & 8 & No & F & Yes & No \\
        \hline

    \end{tabular}
    \vspace{-3mm}
\end{table}

==> old/solution.tex <==
\section{Solution}\label{sec:solution}

{\bf Test for Heterogeneity:}
Using the learned rules, we partition the space into two parts - part 1 and part 0. If the treatment effects are different in these two parts of the space then the following quantity will be large otherwise it will be small.
\begin{equation}\label{eq:test}
    T = \frac{\overline{\tau}_{1}-\overline{\tau}_{0}}{Var(\tau)(1/N^2_1 + 1/N^2_0)}
\end{equation}
Using our example, if we learn the rule that every node which is part of a triangle belongs to part 1 and all the other nodes belong to part 0, then we can test if triangles are effect modifiers (i.e. they cause the treatment effects to change) or not using the equation~\ref{eq:test}.

{\bf The na\"ive approach:} 
The input is the social network graph $G = (V,E)$ and the treatment effect of each unit $u_i$ and the output is the maximum pattern $P$ such that there is a distinguishing explanation pattern. 
% The algorithm examines every size $s$ from $n-1$ to $3$ where $|V| = n$, and for all graphs $G_v$ of size $s$ that include $v \in S$, check if there exists a pattern-preserving isomorphism $f$ from every $v \in S$ to every $u \in S$.
The algorithm examines every size $s$ from $n-1$ to $3$ where $|V| = n$, and for all graphs $G_v$ of size $s$ that include $v \in S$, check if there exists a pattern-preserving isomorphism $f$ mapping every $v \in S$ to every $u \in S$ and there is no pattern-preserving isomorphism mapping $v \in S$ to any $u \in V\setminus S$.


{\bf Improvements:} 
\begin{itemize}
    \item Only inspect interesting patterns (cliques of various sizes, paths to contral nodes, etc.)
    \item Use graph simulation \cite{SunWWSL12,MaCFHW11,Fan12} instead of graph isomorphism to test matches to the pattern
    \item Prioritize finding common covariates first and then consider common patterns as the former is more efficient
\end{itemize}


==> old/to_do.tex <==
\section{To Do}

\begin{itemize}
\color{red}{
    \item Research track submissions are limited to nine (9 pages), including references, must be in PDF and use ACM Conference Proceeding templates. An additional two pages of supplemental material focused on reproducibility can be provided. Additionally, proofs and pseudo-code that could not be included in the main nine-page manuscript may also be included in the two-page supplement.
    \item Refine what we want to explain. Currently drawing on \cite{RoyS14}
    \item The idea of influence can be adopted from \cite{0002M13}, where it is defined as the normalized difference between the result with the set of tuples that satisfies the predicate and the result without it
    \item Start with an algorithm for matchings
    \item use DBToaster \cite{KochAKNNLS14} for IVM
    \item Use the graph structure to identify influential tuples by backtracking from the nodes that are connected to $Y$ nodes
    \item How to compute the influence of a set of tuples for the explanation efficiently?
    \begin{itemize}
        \item Using influence functions may give a way of efficiently computing the influence of the tuples in the regression part \cite{WuF0W20,KohL17}. In \cite{WuF0W20} the author convert the provenance into a probabilistic polynomial and then into a differentiable function that expresses the influence function
        \item The provenance-based model for incremental view maintenance when the view is generated by regression \cite{WuTD20} is less suitable for this use, since it only deals with the removal of data points and not with changing them
        % This concept allows for efficient re-training of the regression model after deleting some training data points. The idea is to represent the process of regression as a provenance polynomial and when a data point is deleted, change the polynomial so that its annotation becomes 0.
    \end{itemize}
    % \item For influence functions, how to connect to the database tuples? using provenance first and then influence function for every row of the unit table?
    % \item Q: What is the training set of the regression that computes the ATE? each unit table row is a data point?
    % \item If using influence functions, look at the influence of change in a set of data points
    \item Another explanation could be a pointing at or correcting the embedding functions that cause the result to be wrong according to the user, similar to \cite{ChapmanJ09}. 
    \item Questions we want to answer:
    \begin{itemize}
        \item Can we divide the units according to treatment effect? or for example, what set of units is most influential in the ATE being so high/low? (explained by the decision tree)
        \item What is the part of the database (source tuples) that influences the ATE (being so high/low)? or what is the most influential covariate set over the ATE being so high/low?
        \item The explanations we give are a generalization of structural equivalence \cite{wasserman1994social,sailer1978structural}.
        \item Suggestion for paper organization: 1. explanations - max common subgraph, 2. max common distinguishing subgraph, 3. max common distinguishing subgraph with common covariates ($+$ neighbors common covariates?)
    \end{itemize}
    \item As opposed to \cite{lee2020causal,athey2016recursive}, we assume the units are part of a social network and thus the structure of the network itself may be an effect modifier
    \item Graph pattern matching may be relevant \cite{SunWWSL12,MaCFHW11,Fan12}
    }
\end{itemize}

==> theory.tex <==
\section{Guarantees of \prob}\label{sec:theory}
In this section discusses the identifiability of the causal effects of interest using the observed variables and the consistency of the test statistic from a theoretical stand-point. 
% Further, we prove few desired properties of our test statistic.

First, we prove that the conditional average treatment effect of interest are identifiable in terms of observables -- $\set{X},\set{Y},\set{T}$ and $\set{E}$. This is important to ensure that we design a method that can estimate the treatment effect using the finite data.

\begin{theorem}[Identification of causal effects]\label{thm:identify}
The causal average treatment effect $\tau(\set{X}_i, \{\set{X}_j\}_{v_j\in \set{V}_{\set{G}_i}\setminus\{v_i\}}, \set{E}_{\set{G}_i}) = E[Y_i(1) - Y_i(0) | \set{X}_i, \{\set{X}_j\}_{v_j\in \set{V}_{\set{G}_i}\setminus\{v_i\}}, \set{E}_{\set{G}_i}]$ is identified as a function of observed variables $\set{X},\set{Y},\set{T}$ and $\set{E}$.
\end{theorem}
% \textbf{Proof.} Using the structural equation for $Y$, we know that potential outcome 
% \begin{equation*}
%     Y_i(t) = \phi_Y\left(\set{X}_i, \{\set{X}_j\}_{v_j\in \set{V}_{\set{G}_i}\setminus\{v_i\}}, \set{E}_{\set{G}_i}, t \right) + \epsilon^Y_i.
% \end{equation*} 
% Thus, if $T_i=t$ then $Y_i(t) = Y_i$ by definition.
% Without loss of generality, let's assume $T_i=1$, then 
% \begin{multline*}
%     E[Y_i(1) | \set{X}_i, \{\set{X}_j\}_{v_j\in \set{V}_{\set{G}_i}\setminus\{v_i\}}, \set{E}_{\set{G}_i}] \\= E[Y_i | \set{X}_i, \{\set{X}_j\}_{v_j\in \set{V}_{\set{G}_i}\setminus\{v_i\}}, \set{E}_{\set{G}_i}, T_i=1].
% \end{multline*}
% By assumption A.4. 
% \begin{multline*}
%     E[Y_i | \set{X}_i, \{\set{X}_j\}_{v_j\in \set{V}_{\set{G}_i}\setminus\{v_i\}}, \set{E}_{\set{G}_i}, T_i=1]\\ = \phi_Y(X_i,\{X_j\}_{j\in N_i\setminus\{i\}}, EN_i, T_i).
% \end{multline*}
% Now, by positivity assumption (equation~\ref{eq:assumption_positivity}). $\exists k$ such that $T_k = 1-T_i$, $\set{X}_i=\set{X}_k$, $\omega_i=\omega_k$ and $\eta_i=\eta_k$.\\ Further, by summarizability assumptions (equation~\ref{eq:assumption_summary}) and A.4. 
% \begin{multline*}
% E[Y_i(0) | \set{X}_i, \{\set{X}_j\}_{v_j\in \set{V}_{\set{G}_i}\setminus\{v_i\}}, \set{E}_{\set{G}_i}]\\=E[Y_i(0) |\set{X}_i, w_i, \eta_i] = \phi_Y(\set{X}_i, w_i, \eta_i, 0)
% \end{multline*}
% Thus, following the argument,
% $$\phi_Y(\set{X}_i, w_i, \eta_i, 0) =
% \phi_Y(\set{X}_k, w_k, \eta_k, 0)$$
% By assumption A.4.
% \begin{multline*}
% \phi_Y(\set{X}_k, w_k, \eta_k, 0) \\= E[Y_k(0) | X_k,w_k, \eta_k]=E[Y_k| X_k,w_k, \eta_k,T_k=0]
% \end{multline*}
% Hence,
% \begin{equation*}
%     \tau_i = E[Y_i| \set{X}_i,w_i, \eta_i,T_i=1]-E[Y_k| \set{X}_k,w_k, \eta_k,T_k=0]
% \end{equation*}
% such that $Z_k = 1-Z_i$, $X_i=X_k$, $w_i=w_k$ and $\eta_i=\eta_k$.
% The above proof proves that the conditional average treatment effect of interest is identifiable in terms of the observables.

Now we show that if we consistently estimate the treatment effects then the test is consistent under null, 
% In other words, with large enough sample size the test type 1 error is low diminishes. 
i.e., the type 1 error of our test \cite{?} \amir{citation for type 1?} diminishes as the size of the data gets larger. 
% We perform a corresponding sample size study in Section~\ref{sec:experiments} using the synthetic data with known ground truth data-generative procedure.

\begin{theorem}[Consistency of \prob\ under null]\label{thm:consistency}
Given a consistent estimator of conditional average treatment effects and average treatment effects, and $I_0=0$, the test statistic $\widehat{\is}_W$ is asymptotically consistent under null i.e. if feature W is not an effect modifier then $\widehat{\is}_W \to 0$ as $n \to \infty$.
\end{theorem}

% \textbf{Proof.} 
% As the causal effect estimator is consistent, we know that $\widehat{\bar{\tau}} \to \bar{\tau}$ and $\widehat{\tau}(w) \to \tau(w)$ when $n\to\infty$. If feature $W$ is not an effect modifier then $(Y(1) - Y(0)) \perp W$. Hence, $E[Y(1) - Y(0)| W=w] = E[Y(1) - Y(0)]$ for all $W=w$. Thus, $\widehat{\ds}_W \to 0$ as $n \to \infty$. This further implies $\widehat{\is}_W\to 0$ as $n \to \infty$. Hence, the test statistic is consistent under null.

% \textbf{Th.3.} $\is_H$ is
% \begin{itemize}
%     \item Scale Invariant
%     \item Size Invariant
%     \item Monotonic with level of Heterogeneity 
% \end{itemize}
% \textbf{Proof.} Same proof as in the Higgins and Thompson paper \cite{higgins2002quantifying}!

